Bounded-degree Low Rank Parity Check Codes

Low-rank parity-check (LRPC) codes are the rank-metric analogue of low-density parity-check codes and they found important applications in code-based cryptography. In this paper we investigate a sub-family of LRPC codes, which have a parity-check matrix defined over a subspace $\calV_{\alpha,d}=\Span{\Fq}{1,\alpha, \ldots, \alpha^{d-1}}\subsetneq \Fqm$, where $\Fqm$ is the finite field of $q^m$ elements and $d$ is a positive integer significantly smaller than $m $; and they are termed bounded-degree LRPC (BD-LRPC) codes. These codes are the same as the standard LRPC codes of density $2$ when the degree $d=2$, while for degree $d>2$ they constitute a proper subset of LRPC codes of density $d$. Exploiting the structure of $\calV_{\alpha,d}$, the BD-LRPC codes of degree $d$ can uniquely correct errors of rank weight $r$ when $n-k \geq r + u$ for certain $u \geq 1$, in contrast to the condition $n-k\geq dr$ required for the standard LRPC codes. This underscores the superior decoding capability of the BD-LRPC codes. Moreover, as the code length $n\rightarrow \infty$, when $n/m\rightarrow 0$, the BD-LRPC codes with a code rate of $R=k/n$ can be uniquely decodable with radius $\rho=r/n$ approaching the Singleton bound $1-R$ by letting $\epsilon=u/n\rightarrow 0$; and when $n/m$ is a constant, the BD-LRPC codes can have unique decoding radius $\rho = 1-R-\epsilon $ for a small $\epsilon$, allowing for $\rho>(1-R)/2$ with properly chosen parameters. This superior decoding capability is theoretically proved for the case $d=2$ and confirmed by experimental results for $d>2$.

==> parts/MonomialLRPC.tex <==
\section{LRPC code of density $>2$}

\iffalse
We already observed that any LRPC code of density $2$ has a parity-check matrix in $\calV_{\alpha,2}$ for some $\alpha \in \Fqm \setminus \Fq.$
Let $\calE \subseteq \Fqm$ be a small subspace and $\calS \subsetneq \calV_{ \alpha,2}.\calE$, if we can expand $\calS$ doing the product with $\calV_{\alpha,t}$ obtaining 
$$
    \calV_{\alpha, t}.\calS \subseteq \calV_{\alpha, t + 1}.\calE.
$$
The key observation is that the dimension of the first subspace can be as big as $t\dim(\calS)$ while the second is at most $(t+1)\dim(\calE)$.
This means that, whenever $\dim(\calS) > \dim(\calE)$, the first subspace has the potential to grow faster than the second and eventually reach it.

Inspired by this result, we aim is to find an expansion function that is faster on a subspace $\calS \subsetneq \calH.\calE$ than it is on $\calH.\calE,$ where $\calH \subseteq \Fqm$ is the support of a parity-check matrix defining an LRPC code.

In the rest of this section, we will describe an expansion that can be seen as the natural generalization of what we did for the case $\calH = \calV_{\alpha,2}.$
An interesting research problem would be to find a better expansion than the one proposed in this paper.
Another interesting result would be to find an expansion that works well for some particular construction of supports like we did for the case $\calH = \calV_{\alpha,d}.$ 
\fi

We already shown how, asymptotically, an LRPC code of density $2$ can be uniquely decoded up to the singleton bound.
In this section we will try to generalize this result for any LRPC code of density $l+1 > 2$.

Let $\calC$ be an LRPC code of density $l+1.$ 
This code will be defined by a parity-check matrix $H \in \Fqm^{(n-k)\times n}$ with support $\calH = \Span{\Fq}{H}$ of dimension $\dim(\calH) = l+1.$
Let $(a_1, \ldots, a_{l+1}) \in \Fqm^l$ be a basis of $\calH$, without loss of generality, we can consider the support $\calH' = a_1^{-1} \calH = \Span{\Fq}{1, \alpha_1, \ldots, \alpha_l},$ where $\alpha_i = a_1^{-1} a_{i+1}.$
The matrix $H' = a_1^{-1}H$ has support $\calH'$ and it is a parity-check matrix of the same code $\calC.$

Thanks to this observation we can naturally extend Definition \ref{Def_Vd} for $\balpha \in \Fqm^l.$
\begin{definition}\label{Def_Vd_multi}
    Let $\Fq[x_1, \ldots, x_l]$ be the ring of polynomials over the field $\Fq$ in $l$ variables.
    Consider $p \in \Fq[x_1, \ldots, x_l]$ and $\balpha \in \Fqm^l$, we denote by $p(\balpha) = p(\alpha_1, \ldots, \alpha_l) \in \Fqm$ the evaluation of $p$ in $\balpha = (\alpha_1, \ldots, \alpha_l).$
    
    For a given integer $d,$ we can define the \textbf{bounded degree subspace} generated by $\balpha$ of degree $d$ as the subspace given by the evaluation in $\balpha$ of all the polynomials of degree strictly smaller than $d.$
    This subspace will be denoted by
    $$
        \calV_{\balpha,d} = \{p(\alpha_1, \ldots, \alpha_{l}) \mid p \in \Fq[x_1, \ldots, x_l], \deg(p) < d \}.
    $$
    A basis of $\calV_{\balpha,d}$ is given by the evaluation in $\balpha$ of all the monomials of degree strictly smaller than $d$ which we will indicate by 
    $$
        \Mon(\balpha, d) 
        =
        \left\{ \prod_{i=1}^{l} \alpha_i^{j_i} \mathrel{\Big|} \sum_{j=1}^l j_i < d \right\}.
    $$
\end{definition}
For $l=1$, Definition \ref{Def_Vd_multi} coincide with Definition \ref{Def_Vd}.
This family of subspaces will follow a result which is the analogue of Lemma \ref{lm:V+aV}.
\begin{lemma}\label{lm:V+aV_l}
    For any $\balpha \in \Fqm^l$ and $i \in [m]$, we have $\dim(\calV_{\balpha,i}) \leq \min\{\binom{l + i -1}{l},m \},$ moreover
    \begin{equation}\label{eq:i.j=i+j-1_l}
         \calV_{\balpha,i}.\calV_{\balpha,j} = \calV_{\balpha,i+j-1},
    \end{equation}
    in particular, for $j=2,$ we have
    \begin{equation} \label{eq:V+aV}
        \calV_{\balpha,i+1} =  \calV_{\balpha,i}.\calV_{\balpha,2} = \calV_{\balpha,i} + \alpha_1 \calV_{\balpha,i} + \ldots + \alpha_l \calV_{\balpha,i}.
    \end{equation}
\end{lemma}
\begin{proof}
    From Definition \ref{Def_Vd_multi}, we have that 
    $$
        \dim(\calV_{\balpha, i}) \leq |\Mon(\balpha,i)|.
    $$
    There are $|\Mon(\bx,i)| = \binom{l+i-1}{l}$ monomials of $l$ variables of degree strictly less than $i.$ 
    This gives us the inequality 
    $$
        \dim(\calV_{\balpha, i}) \leq |\Mon(\balpha,i)| \leq |\Mon(\bx,i)|,
    $$ 
    it follows that $\dim(\calV_{\balpha,i}) \leq \min\{\binom{l + i-1}{l},m \}.$

    For the second part, consider $i, j \in [m]$.
    A basis of $\calV_{\balpha,i}$ is given by $\Mon(\balpha,i)$ and a basis of $\calV_{\balpha,j}$ is given by $\Mon(\balpha,j).$
    Any monomial of degree strictly less than $i+j-1$ can be expressed as the product of to monomials of degree strictly less than $i-1$ and $j-1$ then $\calV_{\balpha,i + j -1} \subseteq \calV_{\balpha,i}.\calV_{\balpha,j}.$
    On the other hand, let $p_i \in \Mon(\balpha,i)$ and $p_j \in \Mon(\balpha,j)$ of degree $\deg(p_i) = d_i < i$ and $\deg(p_i) = d_j < j$ it is straight forward that $\deg(p_ip_j) \leq d_i+d_j < i + j - 1,$ from which follows the result.

    The subspace $\calV_{\balpha,i}.\calV_{\balpha,2}= \calV_{\balpha,i+1}$, has a basis given by $\Mon(\balpha,i+1).$ 
    Notice that $\Mon(\balpha,i+1) = \Mon(\balpha,i) \cup \alpha_1\Mon(\balpha,i) \cup \ldots \cup \alpha_l\Mon(\balpha,i)$ is a basis of $\calV_{\balpha,i} + \alpha_1 \calV_{\balpha,i} + \ldots + \alpha_l \calV_{\balpha,i}$.
    \qed
\end{proof}
Contrary to Lemma \ref{lm:V+aV}, we cannot give a necessary and sufficient condition on $\balpha \in \Fqm^l$ for which $\dim(\calV_{\balpha,i}) = \min\{\binom{l + i -1}{l}, m\}$, for small $i,l$ and $m$ sufficiently large we can assume that equality holds in most of the cases. 

We already discussed how any LRPC code of density $l+1$ admits a parity-check matrix having support $\calH = \Span{\Fq}{1, \alpha_1, \ldots, \alpha_l} = \calV_{\balpha, 2}$ for some $\alpha_1,\ldots, \alpha_l \in \Fqm.$
If we consider $\calE \subset \Fqm$ to be an $\Fq$-linear subspace of dimension $r$ we have that $\dim(\calV_{\balpha, 2}.\calE) \leq \binom{l+2-1}{l}r = (l+1)r.$
If we consider $\calS \subsetneq \calV_{\balpha, 2}.\calE,$ we can apply the expansion given by the product with $\calV_{\balpha, t}$ on both $\calS$ and $\calV_{\balpha, 2}.\calE.$
Suppose $\dim(\calS) = (n-k) < (l+1)r,$ the dimension of $\calV_{\balpha, t}.\calS$ is upper bounded by $\binom{l + t -1}{l}(n-k).$
On the other hand $\calV_{\balpha, t}.\calS \subseteq \calV_{\balpha, t+1}.\calV_{\balpha, 2}.\calE$ which has dimension at most $\binom{l + t }{l}r.$
It can happen that, for $t$ sufficiently large 
\begin{equation}\label{eq:key_dim_l}
    \binom{l + t - 1}{l}(n-k) \geq \binom{l + t}{l}r
\end{equation}
which is satisfied if $n-k> \frac{l+t}{t} r.$
If we consider the density to be $d=l+1$ this inequality becomes $(n-k) \geq  \frac{d+t-1}{t} r$ which is exactly the same as for LRPC codes of density $2$ or CP-LRPC of degree $d.$ 
Asymptotically this inequality will give the same bound $R \leq 1 - \rho.$ The main difference is that, $m \geq \binom{l + t}{l}r$  is considerably larger than it was for LRPC of density $2$ or CP-LRPC of degree $d$.
This will make this approach impractical for large values of $t$ or $l$.

Contrary to the case $l=1,$ it is much harder to predict how the two subspaces will expand.
The choices of $\alpha_1,\ldots, \alpha_l$ will affect heavily affect the dimension of $\calV_{\balpha,t}$.
For example, suppose $l=2$ and $\alpha_2 = \alpha_1^2 + 1$, we will have that 
$$
    \calV_{\balpha,3} = \Span{\Fq}{1,\alpha_1, \alpha_1^2,  \alpha_1^3, \alpha_1^4}
$$
which is at most of dimension $5$ instead of $6$ as we could expect.
If we continue, for $t = 4$ we have 
$$
    \calV_{\balpha,4} = \Span{\Fq}{1,\alpha_1, \alpha_1^2,  \alpha_1^3, \alpha_1^4, \alpha_1^5, \alpha_1^6}
$$
which is at most of dimension $6$ instead of $10$ as the theoretical bound.
This is actually an advantage since it means that the product space can grow significantly slower than expected in some cases and this allows to use a smaller value of $m.$

The other problem for $l>1$ is to model when the expansion of $\calS$ does not reach the expanded product space like we did in Section 4. 
This is also related to the maximal size of $t$ we can use.

\iffalse


\begin{lemma}\label{lm:VjViE}
    Let $\alpha\in \Fqm$ and $\calV_{\alpha,d} \subseteq \Fqm$ be defined as in Def. \ref{Def_Vd} and let $\calE \subseteq \Fqm$ be an $\Fq$-linear subspace of $\Fqm$ of dimension $r$.
    Then for any positive integer $i\geq 1$, we have 
    % We have that
    % \begin{equation} \label{eq:VjViE}
    %     \calV_{\alpha,i+j-1}.\calE = \calV_{\alpha, j}.\calV_{\alpha,i}.\calE.
    % \end{equation}
    \begin{equation} \label{eq:ViE_rec}
        \calV_{\alpha,i+1}.\calE = \calV_{\alpha, 2}.\calV_{\alpha,i}.\calE = \calV_{\alpha,i}.\calE + \alpha \calV_{\alpha,i}.\calE.
    \end{equation}
\end{lemma}
% \begin{proof}
%     The product of subspaces is both associative and commutative.
%     Then (\ref{eq:VjVi}) is a direct consequence of Lemma \ref{lm:V+aV}. \qed
% \end{proof}
The dimension of $ \calV_{\alpha,i}.\calE$ is generally upper bounded by $ir$ when the integer $i \leq m/r$.
Consider $\calS = \Span{\Fq}{s_1, \ldots, s_{n-k}} \subsetneq \calV_{\alpha,d}.\calE$ and suppose its dimension is $\dim(\calS) = (n-k) < rd.$
The standard decoding algorithm for LRPC codes would result in a decoding failure. 
The observation in Lemma \ref{lm:VjViE} motivates us to expand $\calS \subsetneq \calV_{\alpha,d}.\calE$ by the product with $\calV_{\alpha,2}.$
This operation gives
$$
    \calV_{\alpha,2}.\calS \subseteq \calV_{\alpha,2}.\calV_{\alpha,d}.\calE = \calV_{\alpha,d + 1}.\calE.
$$
Notice that $\calV_{\alpha,2}.\calS = \calS + \alpha \calS$ might have dimension up to $2(n-k)$ while $\dim(\calV_{\alpha,d + 1}.\calE) \leq (d+1)r.$
When $n-k \geq (d+1)r/2,$ it is likely that
$\calV_{\alpha,2}.\calS = \calV_{\alpha,d + 1}.\calE$ while $\calS \subsetneq \calV_{\alpha,d}.\calE$.
Furthermore, provided that $m$ is sufficiently larger than $r(d+t-1)$, we can continue expanding $\calS$ with $\calV_{\alpha,t}$, $t\geq 2$, which gives
\begin{equation}\label{eq:expansion_at}
     \calV_{\alpha,t}.\calS \subseteq \calV_{\alpha,t}.\calV_{\alpha,d}.\calE = \calV_{\alpha,d +t-1}.\calE.
\end{equation}
In this case we have $\dim(\calV_{\alpha,t}.\calS) \leq t(n-k)$ while $\dim(\calV_{\alpha,t+d-1}.\calE) \leq (d+t-1)r$. Therefore,
if $t(n-k) \geq (d+t-1)r$, it is likely that $\calV_{\alpha,t}.\calS = \calV_{\alpha,d + t - 1}.\calE.$ When this equality is reached, we can recover the error support $\calE$ from $\calV_{\alpha, t}.\calS$ instead of $\calS$ in the original decoding procedure of LRPC codes.















What can we say about more generic LRPC codes of density $D \geq 2$
In a similar fashion of what we did in the previous section let $\alpha, \beta \in \Fqm$ and consider the space
\begin{equation}\label{MonomialSpace_deg1}
    \calV_{\{\alpha,\beta\},2} = \Span{\Fq}{1,\alpha,\beta}.
\end{equation}
Let $A = \{\alpha, \beta\}$ we will use the more compact notation $\calV_{\{\alpha,\beta\},2} = \calV_{A,2}.$
This space can be expanded as follows
\begin{equation}\label{eq:Monomial_exp2}
    \calV_{A,3} = \calV_{A,2} + \alpha \calV_{A,2} + \beta \calV_{A,2} = \Span{\Fq}{1,\alpha,\beta, \alpha^2, \alpha \beta, \beta^2}.
\end{equation}
Notice that $\{1,\alpha,\beta, \alpha^2, \alpha \beta, \beta^2\}$ are all the monomials of degree strictly less than $3$ in the variables $\alpha,\beta$.
For $m$ sufficiently large, with a good probability, the sum of $3$ spaces of dimension $3$ is a space of dimension $9$ while, in (\ref{eq:Monomial_exp2}), we obtain a space a of dimension $6.$

We introduce the notation $\Mon(A, D)$ to indicate the set of all the monomials in $2$ variables of degree strictly less than $D$ evaluated over the $2$ elements of $A.$
Iterating the same expansion we get
\begin{equation}\label{eq:monomial_expi}
    \calV_{A,i} = \calV_{A,i-1} + \alpha \calV_{A,i-1} + \beta \calV_{A,i-1} = \Span{\Fq}{\Mon(A, i)}.
\end{equation}
The number of monomials in $2$ variables of degree strictly less than $i$ is given by $\binom{i-1+2}{2}$, therefore
the space $\calV_{A,i}$ will have at most dimension $\binom{i-1+2}{2}$.

The same idea can be generalized to a subset $A = \{\alpha_1,\ldots, \alpha_f\}$ of $f$ variables.
As before we denote by $\calV_{A,D} = \Span{\Fq}{\Mon(A, D)}$ the subspace generated by the set of all the monomials in $t = |A|$ variables of degree strictly less than $D$ evaluated over the elements of $A.$
The expansion from  $\calV_{A,i-1}$ to $\calV_{A,i}$ will be obtained by
\begin{equation}\label{eq:GenMon_exp}
     \calV_{A,i} = \calV_{A,i-1} + \sum_{i = 1}^f \alpha_i \calV_{A,i-1} = \calV_{A,i}.\calV_{A,2}. 
\end{equation}
The dimension of $\calV_{A,i}$ is upper bounded by $|\Span{\Fq}{\Mon(A, i)}| = \binom{i-1+f}{f}.$  

Similarly to what we have done in the previous section, we can define an LRPC by a parity-check matrix $H$ having rank support $\calV_{A,d}.$
Suppose we received an error $\be$ of rank $r$ of rank support $\calE = \Span{\Fq}{\be}.$
The support of the syndrome $\bs = H \be^\intercal$ is contained in $\calV_{A,d}.\calE$ that has dimension
\begin{equation} \label{Prod_dim_D}
   \dim(\calV_{A,d}.\calE) \leq \binom{d-1+f}{f} r. 
\end{equation}

Let $\calS_0 \subseteq \calV_{A,d}.\calE$ be the rank support of $\bs$ of dimension $n-k$ and suppose that $n-k < \binom{d-1+f}{f} r.$
We can expand $\calS_0$ to $\calS_1 = \calS_0 + \sum_{i = 1}^f \alpha_i \calS_0$ we get that $\calS_1 = \Span{\Fq}{1,\alpha,\beta}.\calS_0$ which will be contained in the product space $\calV_{\alpha,\beta,D+1}.\calE$ of expected dimension at most $\binom{D+3}{2} r.$
In general when we repeat the expansion we get $\calS_t = \calV_{\alpha,\beta,t}.\calS$ while the product space after $t$ expansions becomes $\calV_{\alpha,\beta,D+t}.\calE$.
Assuming that $m$ is very large and the dimension do not collapse, the parameters should satisfy the following
$$
    (n-k) \binom{t + 2}{2} \geq \binom{D+t+2}{2} r.
$$
From which we get 
$$
    R \leq 1 - \frac{(D+t+2)(D+t+1)}{(t+2)(t+1)} \delta. 
$$

Asymptotically also these codes can achieve $R \leq 1 - \delta.$

\begin{remark}\label{rm:LRPC_3}
    An LRPC code of density $3$ can be considered as a particular case of what we just described.
\end{remark}
Let $\Span{\Fq}{a,b,c}$ be the support of $H \in \Fqm^{(n-k) \times n}$ the parity-check matrix of an LRPC code of density $3$.
Then we can consider the equivalent matrix $H' = (a^{-1}) H$ we have that 
$$
    \Span{\Fq}{H'} =  a^{-1} \Span{\Fq}{H} = \Span{\Fq}{1, a^{-1} b, a^{-1} c} = V_{\alpha, \beta ,1}
$$
where $\alpha = a^{-1} b, \beta = a^{-1} c.$

\subsection{A new algorithm for LRPC codes}
What we saw in Remark \ref{rm:LRPC_2} and Remark \ref{rm:LRPC_3} suggests a to further generalize the expanding procedure to any $LRPC$ code of small density $d$.

Let $A = \{\alpha_1, \ldots, \alpha_d \} \subset \Fqm$ such that $\calA := \Span{\Fq}{A}$ is an $\Fq$-linear subspace of dimension $d$.
We define the space $\calV_{A,D} = \Span{\Fq}{\Mon(A,D)}$ where $\Mon(A,D) =  \{\prod_{\alpha \in A} \alpha^{d_\alpha} \mid \sum_{\alpha \in A} d_{\alpha} \leq D, 0 \leq d_{\alpha}\}.$
Consider now $H \in \Fqm^{(n-k)\times n}$ the parity-check matrix of an LRPC codes having its support in $\calV_{A,D}$.
Suppose we received an error $\be$ of rank $r$ having support $\calE = \Span{\Fq}{\be}.$
We have that 
\begin{equation} %\label{Prod_dim_D}
   \dim(\calV_{A,D}.\calE) \leq \binom{D+d}{d} r 
\end{equation}
for large values of $m$ we can assume that equality holds.
Suppose the space generated by the syndrome $\calS_0 \subseteq \calV_{A,D}.\calE$ has dimension $n-k < \binom{D+d}{d} r.$
Expanding $\calS_0$ to $\calS_1 = \calS_0 + \sum_{\alpha \in A} \alpha \calS_0$, we have $\calS_1 = \Span{\Fq}{\Mon(A,1)}.\calS_0$ which will be contained in the product space $\calV_{A,D+1}.\calE$ of expected dimension at most $\binom{D+1+d}{d} r.$
If we keep applying the same expansion $t$ times we will have
$$
    \calS_t = \Span{\Fq}{\Mon(A,t)}.\calS_0 \subseteq \calV_{A,D+t}.\calE.
$$
From the expected dimensions of the two spaces, we will get the following conditions on the parameters
$$
    (n-k)\binom{t+d}{d} \leq \binom{D+t+d}{d} r.
$$
From which we obtain $R \leq 1 - \mathrm{Z}(t,d,D) \delta$ where 
$$
    \mathrm{Z}(t,d,D) = \frac{(t+d+1) \cdots (t+d+D)}{(t+1) \cdots (t+D)} = \prod_{i=1}^D \frac{t+d+i}{t+i}
$$
for which $\lim_{t \to \infty} \mathrm{Z}(t,d,D) = 1$.
\color{blue}
    The formula for $\mathrm{Z}(t,d,D)$ can also be expressed as $\prod_{i=1}^D (1 + \frac{d}{t+i})$ from which it is clear that $D=1$ is the optimal choice. 
\color{black}

Similar to what we noticed in in Remarks \ref{rm:LRPC_2}, \ref{rm:LRPC_3}.
We have that an LRPC of density $d$ having support $\Span{\Fq}{H} = \Span{\Fq}{\alpha_1, \ldots ,\alpha_d}$, can be interpreted as a monomial LRPC having parity-check support in $ \calV_{A,1} = \alpha_1^{-1} \Span{\Fq}{\alpha_1, \ldots ,\alpha_d}$ where $A = \{\alpha_1^{-1} \alpha_2,\ldots, \alpha_1^{-1} \alpha_d\}$.

The main drawback of considering larger $d$ is that the dimension of the expanded product space $\calV_{A,D + t}.\calE$ grows very quickly with $t$ while we require $m > \dim(\calV_{A,D + t}.\calE)$.

\color{blue}
We conclude this section with an open problem.
The technique we presented in this paper to improve $LRPC$ codes can be summarized as to find particular small $\Fq$-linear subspaces of $\Fqm$ that do not grow as fast as random subspaces when we consider their product subspace with another space.

Given two $\Fq$-linear subspaces $\calU, \calE \subseteq \Fqm$ such that $\dim(\calV)\dim(\calE) < m$, it can be shown that, with a good probability, $\dim(\calV.\calE) = \dim(\calV)\dim(\calE)$.
In some cases the dimension of the product subspace is slightly smaller than the product of the dimensions.

Starting from $\calE$ we can think about repeating the operation of "multiplying" by $\calV$.
Repeating it $t$ times we obtain the space $\calV^t.\calE$ where $\calV^t$ is the space generated by the generators of $\calV$ multiplied by themselves $t$ times.

More formally, if $\calV = \Span{\Fq}{v_1,\ldots, v_d}$, then $\calV.\calV = \Span{\Fq}{v_i v_j \mid i,j \in [d]}$ and $\calV^t = \Span{\Fq}{v_{i_1} \cdots v_{i_d} \mid i_t,\ldots ,i_t \in [d]}$.
The dimension of $\calV^t$ is therefore at most $\binom{t + d}{d}$ that is the number of possible monomials of homogeneous degree $t$ in $d = \dim(\calV)$ variables.
    
That gives the upper bound $\binom{t + \dim(\calV)}{\dim(\calV)} \dim(\calE)$ to the dimension of $\calV^t.\calE.$
This upper bound is usually also the actual dimension of the subspace.
The same bound is true also for the subspace $\calS \subseteq \calV.\calE$ for which we also have
$\dim(\calS.\calV^t) \leq \binom{t + \dim(\calV)}{\dim(\calV)} \dim(\calS).$
Since $\calS \subseteq \calV.\calE$, we can apply the same expansion on the other side obtaining $\calV^{t+1}.\calE$ of dimension at most $\binom{t + 1 + \dim(\calV)}{\dim(\calV)} \dim(\calE).$

Since $\binom{t + 1 + \dim(\calV)}{\dim(\calV)} \dim(\calS) / \binom{t + \dim(\calV)}{\dim(\calV)} \dim(\calS)$ tend to $1$, when $\dim(S) > \dim(E)$ the expansion usually reach the whole space where it should be.

\color{red}
TODO
Can we generalize those result?
From $\calS \subseteq \calV.\calE$ find other expanding function $f$ such that $f(\calS) = f(\calV).\calE$.
The optimal situation is that those expanding function do not expand too much and expand faster the set $\calS$ than the set $f(\calV).\calE.$
Are the function / space used here optimal?

Notice that if we chose $\calV = \mathbb{F}_{q^{m_1}} \subset \Fqm$ where $\mathbb{F}_{q^{m_1}}$is a proper subfield of $\Fqm$ then let $\alpha \Fqm$ a generator of $\mathbb{F}_{q^{m_1}}$ we have that $\calV.\calE + \alpha \calV.\calE = \calV.\calE$ while $\calS \subseteq \calS + \alpha \calS.$

In general this expansion, after $m_1$ iterations takes $\calS = \Span{\Fq}{s_1,\ldots, s_{n-k}}$ and gives $\Tilde{\calS} = \Span{\mathbb{F}_{q^{m_1}}}{s_1,\ldots, s_{n-k}}$.
The $\Fq$-dimension of $\dim(\Tilde{\calS}) \leq m_1 \dim(\calS)$ and is usually equal.
This seems like a perfect expansion function but it does not work when we want to get $\calE.$
Suppose $\Tilde{\calS} = \calV.\calE$, notice that $\calV.\calE = \Span{\mathbb{F}_{q^{m_1}}}{e_1, \ldots e_r}$, from which we cannot obtain the original $\calE$ using the standard multiply and intersect method.

An interesting way to still use this construction is to use different subfields for different equation. I have already some promising magma results in this direction. 
Are there other interesting construction like that?

\color{black}
\section{pathological $\calS$}
Consider the case $\calS \subseteq \calV.\calE'$ where $\calE' \subsetneq \calE.$
No matter how many times we expand $\calS$ we will end up at best in $\calV^t.\calE'.$
That means we can have $\calS = \calV.\calE'$ of dimension up to $rd-d$ and being able to recover only a partial support $\calE'$.

This is a main limitation of the expansion strategy.
How likely is it that a subspace $\calS$ of dimension $\dim(\calS) < rd - d$ gives us an incomplete support?
What's the theory behind it?

Unfortunately there are other cases apart the one mentioned above where the expansion fails.
Consider for example $\calE= \Span{\Fq}{\varepsilon_1,\ldots, \varepsilon_r}$ while $\calH = \Span{\Fq}{1,\alpha,\ldots, \alpha^d} = \calV_{\alpha,d}$.
A generic element of the base $\calS$ will be of the form $s_i = \sum_{j=0}^d \sum_{k=1}^r \lambda_{i,j,k} \alpha^j \varepsilon_k.$
Suppose that for some $\Bar{k} \in [r]$ we have $\lambda_{i,0,\Bar{k}} = 0$ for all $i \in [n-k]$.
This means that the term $\varepsilon_{\Bar{k}}$ will never appear in any element of the base.
If we multiply each term of the base by $\alpha$ we will never get any of the term $\varepsilon_k$, in particular the monomial  $\varepsilon_{\Bar{k}}$ will not appear in any element of the base of $S + \alpha S$.
Therefore $\varepsilon_{\Bar{k}} \notin S + \alpha S$.
The same is clearly true for all the subsequent expansions leading to $\varepsilon_{\Bar{k}} \notin \calV_{\alpha,t}.\calS \subsetneq \calV_{\alpha, d+t}.\calE.$
In other word the expansion of $\calS$ will never encompass the expansion of $\calE.$

A similar situation appears if the term $\alpha^d \varepsilon_{\Bar{k}}$ is not present in any of the basis elements of $\calS.$
In this case $\alpha^{d+t} \varepsilon_{\Bar{k}} \notin \calV_{\alpha,t}.\calS$ while $\alpha^{d+t} \varepsilon_{\Bar{k}} \in \calV_{\alpha,d+t}.\calE$.
\fi

==> parts/OldSuccessfulExpansion.tex <==
\section{Successful subspace expansion.}\label{sec:Successful}
% In the previous section, we saw how it is possible to  increase the rate of some LRPC codes, while maintaining the same error correction capability.
% This is achieved thanks to an expansion that involves both the support of the syndrome and the product space where it is contained.



For BD-LRPC codes, assume $\calS \subseteq \Fqm$ is the subspace generated by the syndrome $\bs=\be H^\intercal$ and $\calV_{\alpha,d}.\calE \subseteq \Fqm$ is the product space between the parity check matrix support $\calV_{\alpha,d}$ and the error support $\calE.$
In the previous section, we briefly pointed out that we can 
expand $\calS$ and $\calV_{\alpha,d}.\calE$ by 
 the product with $\calV_{\alpha,t}$, for certain integer $t\geq 1$, 
 which leads to 
 $\calV_{\alpha,t}.\calS = \calV_{\alpha,d + t -1}.\calE$ with a high probability.
 In this section, we shall intensively discuss the probability of this equality.

% Unfortunately, what we observed with Magma simulation, is that in some cases this growth was slower than expected.
% In some cases, the co-dimension between $\calV_{\alpha,i}.\calS$ in $\calV_{\alpha,d + i -1}.\calE$ reach a minimum for some $i$ and then is constant for each $j \geq i.$
% In these cases, it does not matter how big is $m$ and how many expansions we do, we will never reach $\calV_{\alpha, j}$, hence we will never recover $\calE.$
 
Consider the space $\calE = \Span{\Fq}{\be}$ with a basis ${\bm\varepsilon} = (\varepsilon_1, \ldots, \varepsilon_r)$ and
$\calS =\Span{\Fq}{\bs}$, where $\bs=(s_1,\dots, s_{n-k})$ is the syndrome. Since $\calS$ is a subspace of the product space $\calV_{\alpha,d}.\calE$, we have
$$
   \calS \subseteq \calV_{\alpha,d}.\calE = \calE + \alpha \calE  + \ldots + \alpha^{d-1} \calE .   
$$
For each $s_i \in \calS$ there exists $(x_{i,1}, \ldots, x_{i,d}) \in \calE^d$ such that $s_i = \sum_{j=1}^d x_{i,j}\alpha^{j-1}.$
Denote by $\ba_d$ the vector $\ba_d = (1,\alpha, \ldots, \alpha^{d-1})$, which is a basis of $\calV_{\alpha, d}$. Then we have $s_i = (x_{i,1}, \ldots, x_{i,d}) \ba_d^\intercal.$
Consider the matrix $X \in \calE^{(n-k) \times d}$ whose $i$-th row is given by $(x_{i,1}, \ldots, x_{i,d})$. This gives 
$$
    \bs^\intercal
    =
    X \ba_d^\intercal.
$$
Let $\bx_j^\intercal \in \calE^{n-k}$ denote the $j$-th column of $X$.
We can expand it to the matrix $X_j \in \Fq^{(n-k) \times r}$ defined as the matrix such that 
$
    X_j \bee^{\intercal} = \bx_j^\intercal.
$
The syndrome $\bs$ can then be obtained as 
\begin{equation}\label{eq:SyndromeSum}
    \begin{pmatrix}
        s_1 \\ \vdots \\ s_{n-k}
    \end{pmatrix}
    =
    X_1 \bee^\intercal + \alpha X_2 \bee^\intercal + \ldots + \alpha^{d-1} X_{d} \bee^\intercal 
\end{equation}
The basis of $\calV_{\alpha,d}.\calE$ is given by 
$
    \ba_d \otimes \bee = 
    (\bee, \alpha \bee, \ldots, \alpha^{d-1} \bee) \in \Fq^{dr},
$ implying
$\calV_{\alpha,d}.\calE = \Span{\Fq}{\ba_d \otimes \bee}.$ Using these notations we have 
\begin{equation}\label{eq:SyndromeAsMatrix}
    \bs^\intercal
    =
    \begin{pmatrix}
        X_1 & \ldots & X_d 
    \end{pmatrix}
    (\ba_d \otimes \bee)^\intercal.
\end{equation}
This equation describes the coordinates of the syndrome with respect to the generator $\ba_d \otimes \bee$ of $\calV_{\alpha,d}.\calE$.
When $\dim(\calS) = \dim(\calV_{\alpha,d}.\calE) = dr$, 
$X_1,\ldots, X_d$ induce a one-to-one correspondence between $\bs$ and $\ba_d \otimes \bee$, thus $\bee$ can be uniquely determined.

Now we consider the cases where $\calS \subsetneq \calV_{\alpha,d}.\calE$ and start with the first expansion.
The expansion is given by $\calV_{\alpha,2} \calS = \calS + \alpha \calS \subseteq \calV_{\alpha,d+1}.\calE.$
Note that $\alpha \bs$ is a generator of $\alpha \calS$ since $\bs$ is a generator of $\calS$.
As in (\ref{eq:SyndromeSum}), we can express $\alpha \bs$ as
\begin{equation}\label{eq:AlphaSyndromeSum}
   \alpha
   \begin{pmatrix}
        s_1 \\ \vdots \\ s_{n-k}
    \end{pmatrix}
    =
    \alpha X_1 \bee^\intercal + \alpha^2 X_2 \bee^\intercal + \ldots + \alpha^d X_d \bee^\intercal 
\end{equation}
Denote $\ba_{d+1} = (1,\alpha, \ldots, \alpha^{d})$. Then
a basis of $\calV_{\alpha,d+1}.\calE$ can be given by $\ba_{d+1} \otimes \bee = (\ba_d \otimes \bee, \alpha^d \bee) \in \Fqm^{(d+1)r}.$
Thus we have
\begin{equation}\label{eq:AlphaSyndromeAsMatrix}
    \alpha \bs^\intercal
    =
    \begin{pmatrix}
        \bzero & X_1 & \ldots & X_d 
    \end{pmatrix}
    (\ba_{d+1} \otimes \bee)^\intercal.
\end{equation}
Combining (\ref{eq:SyndromeAsMatrix}) and (\ref{eq:AlphaSyndromeAsMatrix}) gives the system
\begin{equation}\label{eq:Exp2AsMatrix}
    \begin{pmatrix}
        \bs^\intercal \\
        \alpha \bs^\intercal
    \end{pmatrix}
    =
    \begin{pmatrix}
        X_1 & X_2 & \ldots & X_d & \bzero \\
        \bzero & X_1 & X_2 & \ldots & X_d 
    \end{pmatrix}
    (\ba_{d+1} \otimes \bee)^\intercal.
\end{equation}
We can similarly extend \eqref{eq:Exp2AsMatrix}  for the general expansion $\calV_{\alpha,t} \calS = \calV_{\alpha,d+t-1}.\calE.$
In this case $\ba_{d+t} \otimes \bee$ is a basis of $\calV_{d+t-1}.\calE$ and the coordinates of $(\ba_t \otimes \bs)^\intercal = (\bs, \alpha \bs, \ldots \alpha^{t-1} \bs)^\intercal$ can be expressed as
\begin{equation} \label{eq:ExpAsMatrix}
    \begin{pmatrix}
       \bs^\intercal \\ \alpha \bs^\intercal \\ \vdots \\ \alpha^{t-1} \bs^\intercal
    \end{pmatrix}
    =
    \begin{pmatrix}
        X_1 & X_2 & \cdots & X_d     & 0   & \cdots & 0 \\
        0   & X_1 & X_2 & \cdots & X_d & \cdots & 0 \\
        \vdots   &  & \ddots & \ddots  &  & \ddots & \vdots \\
        0   & \cdots &  0 & X_1  & X_2 & \cdots & X_d 
    \end{pmatrix}
    \begin{pmatrix}
        \bee^\intercal \\ \alpha \bee^\intercal \\ \vdots \\ \alpha^{d+t-2} \bee^\intercal 
    \end{pmatrix}.
\end{equation}
The above expansion is considered successful when
$\calV_{\alpha,t} \calS = \calV_{\alpha, d+t-1}.\calE$, which
can be stated in terms of bases as $$\Span{\Fq}{\ba_t \otimes \bs} = \Span{\Fq}{\ba_{d+t-1} \otimes \bee}.$$

Let $M_t$ be the matrix in (\ref{eq:ExpAsMatrix}), which has $(n-k)t$ rows and $(d+t-1)r$ columns.
If $M_t$ has full rank $rd$, then there will be an invertible square sub-matrix $\hat{M_t}$ of order $(d+t-1)r$ in $M_t$ and a corresponding sub-vector $\hat{\bs} \in \Fq^{(d+t-1)r}$ such that $\hat{\bs}^\intercal = \hat{M_t} (\ba_{d+t-1} \otimes \bee)^\intercal.$
This implies 
\begin{equation}\label{eq:se}
    \hat{M_t}^{-1}\hat{\bs}^\intercal  =  (\ba_{d+t-1} \otimes \bee)^\intercal.
\end{equation}
That is to say, all the entries of $(\ba_{d+t-1} \otimes \bee)$ can be obtained as $\Fq$-linear combinations of entries in $\hat{\bs}.$
In this case, we have that $\Span{\Fq}{\ba_{d+t-1} \otimes \bee} \subseteq \Span{\Fq}{\hat{\bs}}$ 
while $\Span{\Fq}{\hat{\bs}} \subseteq \Span{\Fq}{\ba_t\otimes\bs},$
from which $\Span{\Fq}{\ba_{d+t-1} \otimes \bee} = \Span{\Fq}{\ba_t\otimes\bs}.$

\color{black}
% The entries of the matrices $X_i \in \Fq^{(n-k)\times r}$ in (\ref{eq:ExpAsMatrix}) depend on the syndrome $\bs.$ 
% Heuristically these matrices behave as random matrices uniformly drawn from $\Fq^{(n-k)\times r}$.
% We shall use this assumption and establish a necessary and sufficient condition for the matrix $M_t$ to have full rank $(d+t-1)r.$
% The assumption that $X_i$ follows uniform distribution over $\Fq^{(n-k)\times r}$ can be justified under certain conditions on $H$, which is discussed in Lemma \ref{lm:SyndromeUniform}.

Observe that one necessary (but not sufficient) condition for $M_t$ to be of full rank $(d+t-1)r$ is that $(n-k)t \geq (d+t-1)r$ and $\Rank(X_1) = \Rank(X_d) = r.$ The derivation of a necessary and sufficient condition is relatively complicated for general $d$.
So we start by considering the case $d=2$, which exhibits our approach for the general case. 

In order to satisfy $(n-k)t \geq (d+t-1)r$, we need  $(n - k) \geq (1+\frac{d-1}{t})r$, which implies $n-k\geq r + \frac{r}{t}$ for $d=2$.
Denote $u = n-k-r$. Then we have $u \geq r/t.$
In the following, we will show that the probability that $M_t$ has full rank $(t+1)r$ for $t = r-1$, is in the order of $1 - q^{-u + 1}.$
% \begin{theorem}\label{th:d2rate}
%     Let $\calC \subseteq \Fqm^n $ be an LRPC code of density $2$. That is an LRPC code that admits a parity check matrices $H$ of support $\Span{\Fq}{H} = \Span{\Fq}{1,\alpha}$ for some $\alpha \in \Fqm.$ 
%     Let $R$ be the rate of $\calC$ and let $\delta$ be the error rate.
%     Provided that $m$ and $n$ are sufficiently large, it is possible to correct an error of rank $\delta n$ with failure rate in the order of $q^{-u}$ with a rate
%     $$
%         R \leq 1 - \delta - u/n.
%     $$
% \end{theorem}

From \eqref{eq:ExpAsMatrix} the matrix $M_t$ for $d=2$ is given by
\begin{equation}\label{eq:Mt2}
    M_t 
    =
    \begin{pmatrix}
        X_1 & X_2 &        &        &       \\
            & X_1 & X_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & X_1    & X_2   
    \end{pmatrix}
    \in \Fq^{(r+u)t \times (t+1)r}.
\end{equation}
% Each of the matrices $X_1, X_2 \in \Fq^{(r+u)\times r}$ will be of full rank $r$ with probability $\prod_{i= 0}^{r-1} (q^{r+u} - q^i)/q^{r(r + u)} \approx 1 - q^{(r-1)(r+u)}(q^r-1)/(q-1) q^{-r(r+u)} \approx 1 - q^{-u}.$
% These conditions are unfortunately not enough to guarantee that $M_t$ is of full rank.
Suppose that $X_1,X_2$ are of full rank $r$, we can analyze the problem as follows.
Firstly, choose a permutation matrix $P_0$ such that 
$P_0(X_1,X_2) = \begin{psmallmatrix} Y_1 & Y_2\\ Z_1 & Z_2 \end{psmallmatrix}$,
where $Y_1 \in \Fq^{r \times r}$ is an invertible matrix and $Z_1, Z_2 \in \Fq^{u \times r}.$ 
Iteratively applying $P_0$ on $X_1, X_2$ in $M_t$, we obtain
\begin{equation}\label{eq:Mt2_stairs}
M_t\rightarrow    P M_t 
    =
    \begin{pmatrix}
        Y_1 & Y_2 &        &        &       \\
            & Y_1 & Y_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & Y_1    & Y_2   \\
        Z_1 & Z_2 &        &        &       \\
            & Z_1 & Z_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & Z_1    & Z_2      
    \end{pmatrix}
    \in \Fq^{(r+u)t \times (t+1)r}.
\end{equation}
It is clear that $M_t$ has full rank if and only if $PM_t$ has full rank.
% In particular, since $X_1$ is of full rank $r$, there exists a permutation $P$ such that $Y_1 \in \Fq^{r \times r}$ is invertible and $Z_1 \in \Fq^{u \times r}.$
% The same permutation will split $X_2$ into $Y_2 \in \Fq^{r\times r}$ and $Z_2 \in \Fq^{u \times r}.$
Since $Y_1$ is invertible, there exists a matrix $A \in \Fq^{r \times r}$ such that $Y_1 A = -Y_2$. Moreover, we have $\RowSpan(A) = \RowSpan(Y_2).$
We can use this relation to further transform $M_t$ as follows
\begin{equation}
M_t\rightarrow PM_t=\begin{pmatrix}
        Y_1 & Y_2 &        &        &       \\
            & Y_1 & Y_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & Y_1    & Y_2   \\
        Z_1 & Z_2 &        &        &       \\
            & Z_1 & Z_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & Z_1    & Z_2      
    \end{pmatrix} \rightarrow
    \begin{pmatrix}
        Y_1 &     &        &        &       \\
            & Y_1 & Y_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & Y_1    & Y_2   \\
            & Z   &        &        &       \\
            & Z_1 & Z_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & Z_1    & Z_2      
    \end{pmatrix},
\end{equation}
where $Z = Z_1 A + Z_2.$
By iteratively applying this reduction $t$ times to eliminate all the instances of $Y_2$,
we have the following elementary transformations on $M_t$:
\begin{equation}\label{eq:redMt2}
M_t \rightarrow PM_t \rightarrow    \Tilde{M_t}
    = 
    \begin{pmatrix}
        Y_1 &     &        &        &           \\
            & Y_1 &        &        &           \\
            &     & \ddots &        &           \\
            &     &        & Y_1    &           \\
            % &     &        &        & ZA^{t-1}  \\
            % &     &        &        & ZA^{t-2}  \\
            % &     &        &        & \vdots    \\
            &     &        &        & \Tilde{Z}     
    \end{pmatrix} \text{ with } \Tilde{Z}=\begin{pmatrix}
    ZA^{t-1} \\ ZA^{t-2} \\ \vdots \\ Z
    \end{pmatrix}.
\end{equation}
% Denote by $\Tilde{Z}  
% $the lower part of $\Tilde{M}_t$ formed by $Z, ZA, \dots, ZA^{t-1}$.
It is readily seen that 
$$
    \Rank(M_t) =\Rank(\Tilde{M_t}) = t \Rank(Y_1) + \Rank(\Tilde{Z}) = tr + \Rank(\Tilde{Z}).
$$
Hence the probability of $\Rank(M_t)= (t+1)r$ is the same as the probability probability that 
$\RowSpan(\Tilde{Z}) = \Fq^r$ and $\Rank(Y_1) = r$.
From the definition of $\Tilde{Z}$, we have 
$$\RowSpan(\Tilde{Z}) = \RowSpan(Z) + \ldots + \RowSpan(ZA^{t-1}) = \Fq^r.$$
Calculating this probability requires a detailed investigation of the relation between rows in the $\RowSpan(ZA^i)$ for $i=0,1,\dots,t-1$. 
Section \ref{sec:ExpRowSub} is dedicated to the calculation of this probability for uniformly distributed $Z$ and $A$.

Recall that $X_1, X_2$ are obtained from the syndrome $\bs$ over $\calE$.
Heuristically $X_1, X_2$ follow a uniform distribution over $\Fq^{(n-k)\times r}$.
This property is theoretically confirmed in the following lemma.
\begin{lemma}\label{lm:SyndromeUniform}
Let the $(n-k)\times n$ matrix $H$ over $\calV_{\alpha,2}$
be decomposed as $H = H_1 + \alpha H_2,$ where $H_1,H_2 \in \Fq^{(n-k) \times n}.$
Let $\calE\subseteq \Fqm$ be an $\Fq$-linear subspace of dimension $r$ such that $\dim(\calV_{\alpha, 2}.\calE) = 2r$.
    If $\Rank \begin{psmallmatrix} H_1 \\ H_2 \end{psmallmatrix} = 2(n-k)$ then, for each $\bs \in (\calV_{\alpha, 2}.\calE)^{n-k}$ the set 
    $$
        \Sol(\bs)=\{\be \in \calE^n \mid H \be^\intercal = \bs^\intercal \}
    $$ 
    has the same cardinality $q^{r(2k-n)}$.
\end{lemma}
\begin{proof}
    If the subspace $\calV_{\alpha,2}.\calE=\Span{\Fq}{1, \alpha}.\calE$ has dimension $2r$, it can be decomposed into the direct sum of $\calE$ and $\alpha \calE.$
    Then the vector $\bs$ can be decomposed into $\bs = \bs_1 + \alpha \bs_2$ where $\bs_1,\bs_2 \in \calE.$
    If there exists $\be \in \calE^n$ such that $H \be^\intercal = \bs^\intercal$, then $H_1 \be^\intercal = \bs_1$ and $H_2 \be^\intercal = \bs_2$.
    We can expand $\bs_1^{\intercal}, \bs_2^\intercal$ into two matrices $X_1, X_2 \in \Fq^{(n-k)\times r}$ such that
    $$
        \bs_1^\intercal = X_1 \begin{pmatrix} \varepsilon_1 \\ \vdots \\ \varepsilon_r \end{pmatrix}, \quad \bs_2^\intercal = X_2 \begin{pmatrix} \varepsilon_1 \\ \vdots \\ \varepsilon_r \end{pmatrix}. 
    $$
    Similarly we can expand $\be^\intercal \in \calE^n$ to a matrix $E \in \Fq^{n \times r}$ such that $\be^\intercal = E (\varepsilon_1, \ldots, \varepsilon_r)^\intercal.$
    We obtain the expanded system 
    \begin{equation}\label{eq:SyndromeUniformExpanded}
        \begin{pmatrix}
            H_1 \\
            H_2
        \end{pmatrix}
        E 
        =
        \begin{pmatrix}
            X_1 \\
            X_2
        \end{pmatrix}
    \end{equation}
    By hypothesis $H' = \begin{psmallmatrix} H_1 \\ H_2 \end{psmallmatrix}$ has rank $2(n-k).$
    Restrict the system (\ref{eq:SyndromeUniformExpanded}) to the $i$-th column of $\begin{psmallmatrix} X_1 \\ X_2 \end{psmallmatrix}$ there are possible $q^{2k - n}$ choices of the $i$-th column of $E$ that will be a solution of the restricted system.
    For each choice of  $\begin{psmallmatrix} X_1 \\ X_2 \end{psmallmatrix}$ there will be $q^{r(2k - n)}$ possible matrices $E$ that satisfy (\ref{eq:SyndromeUniformExpanded}). 
    This is equivalent to say that, for each $\bs \in (\calV_{\alpha, 2}.\calE)^{n-k}$, the set $\Sol(\bs)$ has $q^{r(2k - n)}$ elements.
    % \qed
\end{proof}

From Lemma \ref{lm:SyndromeUniform} one can clearly see that, when $\be$ is uniformly drawn from
$\calE^n$, if $\dim(\calV_{\alpha,2}.\calE) = 2r$,  the matrices $X_1,X_2$ derived from $\bs=\bs_1+\alpha \bs_2$ follow a uniform distribution. Note that the matrix $Z=Z_1A+Z_2$ and $A$  can be deemed to follow a uniform distribution 
over $\Fq$. As a matter of fact, assume $X_2$ in (\ref{eq:Mt2}) is
uniformly drawn from $\Fq^{(n-k) \times r}$. Recall that $\begin{psmallmatrix}
Y_2 \\ Z_2
    \end{psmallmatrix}
    =P_0X_2
    $
    and
$A = -Y_1^{-1} Y_2$. Thus we have
\begin{equation}\label{eq:AZ_uniform}
\begin{pmatrix}
        A \\ Z
    \end{pmatrix} 
    =
    \begin{pmatrix}
        -Y_1^{-1} & \bzero \\
        - Z_1 Y_1^{-1} & I_{u}
    \end{pmatrix}
    \begin{pmatrix}
        Y_2 \\ Z_2
    \end{pmatrix}
    = \begin{pmatrix}
        -Y_1^{-1} & \bzero \\
        - Z_1 Y_1^{-1} & I_{u}
    \end{pmatrix}
    P_0X_2
\end{equation} 
It is readily seen that 
$\begin{psmallmatrix}  A \\ Z \end{psmallmatrix}$ 
has a one-to-one correspondence to the uniformly distributed $X_2$. Therefore,  $\begin{psmallmatrix}  A \\ Z \end{psmallmatrix}$  also follows a uniform distribution.

\smallskip

As it will be shown in Corollary \ref{cor:Pr(C_k^u)} in Section \ref{sec:ExpRowSub}, the probability that a matrix $\begin{psmallmatrix}  A \\ Z \end{psmallmatrix}$ uniformly drawn from $\Fq^{(r+u) \times r}$ leads to $\sum_{i=0}^{r-1} \RowSpan(ZA^{i}) = \Fq^r$ is in the order of $1 - \frac{q^{-u+1}}{q-1}.$ 
At the same time, the probability that a random matrix $X_1$, uniformly chosen in $\Fq^{(r+u)\times r}$, has rank $r$ is given by 
$$
    q^{-(r+u)r}\prod_{i = 0}^{r-1}(q^{r+u} - q^i) \approx 1 - q^{-r-u} \sum_{i=0}^{r-1}q^i  \approx 1 - \frac{q^{-u}}{(q-1)}.
$$
Combining the above analysis, we have the following result:

\begin{proposition}\label{prop:1}
Let $\calC \subseteq \Fqm^n $ be an LRPC code having one 
    parity check matrix $H\in \Fqm^{(n-k)\times n}$ of support $\Span{\Fq}{H} = \calV_{\alpha, 2}$ for some $\alpha \in \Fqm.$ 
    Suppose $\be\in\Fqm^n$ is an error of rank $r$ and denote $\calE=\Span{\Fq}{\be}$
    and $\calS=\Span{\Fq}{\bs}$, where $\bs= \be H^\intercal$. Then, 
    the probability that 
    $\calV_{\alpha, r-1}.\calS = \calV_{\alpha, r}.\calE$ 
    is given by $1- \frac{q+1}{q-1} q^{-u}$, where $u=(n-k)-r$. 
\end{proposition}




% obtain that for an LRPC code $\calC$
% with parity check matrix $H\in \Fqm^{(n-k)\times n}$ having support $\Span{\Fq}{H} = \Span{\Fq}{1,\alpha}$ and an error $\be$ of rank $r$ uniformly drawn from $\calE^n$, 
% under the condition that $(n-k)\geq r + \frac{r}{r-1}$,
% the probability that the syndrome space $\calS$ satisfying 
% $\calV_{\alpha, r-1}.\calS = \calV_{\alpha, r}. \calE$ is in the order of $\frac{q^{-u+1}}{q-1}$.



% \begin{theorem}\label{th:d2rate}
%     Let $\calC \subseteq \Fqm^n $ be an LRPC code having one 
%     parity check matrice $H\in \Fqm^{(n-k)\times n}$ of support $\Span{\Fq}{H} = \Span{\Fq}{1,\alpha}$ for some $\alpha \in \Fqm.$ 
%     For sufficiently large $m$, $n$ and $k< \frac{n}{2}$,
%     an error $\be\in\Fqm^n$ of rank $r\leq \frac{n}{2}$ can be corrected with a failure rate in the order of $\frac{q^{-(u+1)}}{q-1}$, where $u=(n-k)-r$.
% \end{theorem}

% It is now time to give a good reason why $X_1, X_2$ in (\ref{eq:Mt2}) can be considered as independently drawn from a uniform distribution.

% When the conditions of this lemma are satisfied, the matrices in (\ref{eq:Mt2}) can be considered uniformly chosen and independent.
% For these codes we can then rigorously prove that Theorem \ref{th:d2rate}.
% For the other cases it seems fair to assume that the matrices $X_1,X_2$ will still behave like if they were independently uniformly drawn.

% \subsubsection{Consecutive power LRPC codes}
We can now extend our analysis for a general small integer $d$.
A successful expansion is obtained when there exists $t$ such that $\calV_{\alpha,t}.\calS = \calV_{\alpha,d+t-1}.\calE.$
Let $\bee \in \Fqm^{r}$ be a basis of the error support $\calE$ and let $\bs \in \Fqm^{n-k}$ be a basis of the syndrome support.
If we define $\ba_t = (1, \alpha, \ldots, \alpha^{t-1})$, we have that $\calV_{\alpha,t}.\calS = \Span{\Fq}{\ba_t \otimes \bs}$ and $\calV_{\alpha, d+t-1} = \Span{\Fq}{\ba_{d+t-1} \otimes \bee}.$
The syndrome expansion was already modeled in (\ref{eq:ExpAsMatrix}) giving the equation $(\ba_t \otimes \bs)^\intercal = M_t(\ba_{d+t-1} \otimes \bee)^\intercal $ where 
\begin{equation} \label{eq:Mtd}
    M_t
    =
    \begin{pmatrix}
        X_1 & X_2 & \cdots & X_d       &     &        &     \\
            & X_1 & X_2    & \cdots    & X_d &        &     \\
            &     & \ddots & \ddots    &     & \ddots &     \\
            &     &        & X_1       & X_2 & \cdots & X_d 
    \end{pmatrix}.
\end{equation}
When $\Rank(M_t) = (d+t-1)r$, each component of $\ba_{d+t-1} \otimes \bee$ can be expressed as an $\Fq$-linear combination of components of $\ba_t \otimes \bs,$ indicating  $\calV_{\alpha,t}.\calS = \calV_{\alpha,d+t-1}.\calE.$
A necessary but not sufficient condition in order to have full rank is that $\Rank(X_1) = \Rank(X_d)= r.$

Suppose $\Rank(X_1) = r$, as we did for the case $d=2$, we can rearrange the rows of $M_t$ to obtain  the matrix
\begin{equation}\label{eq:Mtd_stairs}
    P M_t
    =
    \begin{pmatrix}
        Y_1 & Y_2 & \cdots & Y_d       &     &        &     \\
            & Y_1 & Y_2    & \cdots    & Y_d &        &     \\
            &     & \ddots & \ddots    &     & \ddots &     \\
            &     &        & Y_1       & Y_2 & \cdots & Y_d \\
        Z_1 & Z_2 & \cdots & Z_d       &     &        &     \\
            & Z_1 & Z_2    & \cdots    & Z_d &        &     \\
            &     & \ddots & \ddots    &     & \ddots &     \\
            &     &        & Z_1       & Z_2 & \cdots & Z_d 
    \end{pmatrix},
\end{equation}
where $Y_i \in \Fq^{r\times r}$ is invertible and $Z_i \in \Fq^{u \times r}.$
Since $Y_1$ is invertible, there exist square matrices  $A_1, \ldots, A_{d-1}$ such that $Y_1 A_{i-1} = -Y_i$. Moreover, these matrices satisfy $\RowSpan(A_i) = \RowSpan(Y_i).$

We can transform $PM_t$ to
\begin{equation}\label{eq:Mtd_1}
    M_t^{(1)}
    =
    \begin{pmatrix}
        Y_1 &     		&        &           	 &     &        &     \\
            & Y_1 		& Y_2    & \cdots    	 & Y_d &        &     \\
            &     		& \ddots & \ddots    	 &     & \ddots &     \\
            &     		&        & Y_1       	 & Y_2 & \cdots & Y_d \\
            & Z_1^{(1)} & \cdots & Z_{d-1}^{(1)} &     &        &     \\
            & Z_1 		& Z_2    & \cdots    	 & Z_d &        &     \\
            &     		& \ddots & \ddots    	 &     & \ddots &     \\
            &     		&        & Z_1       	 & Z_2 & \cdots & Z_d 
    \end{pmatrix},
\end{equation}
where $Z_{i}^{(1)} = Z_1 A_i + Z_{i+1}.$
We can continue reducing the second block with the same matrices $A_1, \ldots, A_{d-1}$.
This will give us the further reduction
\begin{equation}\label{eq:Mtd_2}
    M_t^{(2)}
    =
    \begin{pmatrix}
        Y_1 &     &        		&        &     			 &         &     \\
            & Y_1 &        		&        &     			 &         &     \\
            &     & \ddots      & \ddots   &     & \ddots &     \\
            &     &        		& Y_1    & Y_2 			 & \cdots  & Y_d \\
            &     & Z_1^{(2)} 	& \cdots & Z_{d-1}^{(2)} &     	   &     \\
            &     & Z_1^{(1)}   & \cdots & Z_{d-1}^{(1)} &         &     \\
            &     & \ddots 		& \ddots &     			 & \ddots  &     \\
            &     &        		& Z_1    & Z_2 			 & \cdots  & Z_d 
    \end{pmatrix},
\end{equation}
where $Z_{i}^{(2)} = Z_1^{(1)} A_i + Z_{i+1}^{(1)}$ for $1\leq i<d$ and $Z_{d}^{(1)} = \bzero.$
Let us define $Z^{(j)} \in \Fq^{u \times (d-1)r}$ as $Z^{(j)} = ( Z_1^{(j)} \cdots Z_{d-1}^{(i)})$ and the square matrix $A \in \Fq^{(d-1)r \times (d-1)r}$ as
\begin{equation}
    A =
	\begin{pmatrix}
		A_1 & A_2 & \cdots & A_{d-2} & A_{d-1} 	\\
		I_r &     &        &         &  \bzero  \\
			& I_r &  	   &         &  \bzero  \\
			&	  & \ddots &         &  \vdots  \\
			&     &		   & I_r     & 	\bzero	
		\end{pmatrix}.
\end{equation}
Observe that $Z^{(2)} = Z^{(1)} A$. More generally,
we have $Z^{(j+1)} = Z^{(j)} A$, implying that 
$Z^{(j+1)} = Z^{(1)}A^j$ for $j=1, 2,\dots, t-2$. 
After iterating $t$ times we obtain the matrix
\begin{equation}\label{eq:Mtd_t}
    M_t^{(t)}
    =
    \begin{pmatrix}
        Y_1 &     &        &     &     			  \\
            & Y_1 &        &     &     			  \\
            &     & \ddots &     &     			  \\
            &     &        & Y_1 &  			  \\
            &     &        &     & Z^{(1)}A^{t-1} \\
            &     &        &     & Z^{(1)}A^{t-2} \\
            &     &        &     & \vdots         \\
            &     &        &     & Z^{(1)} 		  
    \end{pmatrix},
\end{equation}
which has the same pattern as in (\ref{eq:redMt2}).
Hence we have
$$
    \Rank(M_t^{(t)}) = t \Rank(Y_1) + \Rank(\Tilde{Z}) =  rt + \Rank(\Tilde{Z}),
$$
where the matrix $\Tilde{Z}$ is defined as 
$$
    \Tilde{Z} 
    =
    \begin{pmatrix}
        Z^{(1)} \\ Z^{(1)} A \\ \vdots \\ Z^{(1)} A^{t-1}
    \end{pmatrix}
    \in \Fq^{ut \times r(d-1)}.
$$
Therefore, the problem of 
considering $\Rank(M_t) = (d+t-1)r$ is equivalent to considering $\Rank(X_1) = r$ and $\Rank( \Tilde{Z}) = r(d-1).$

In order to apply Corollary \ref{cor:Pr(C_k^u)}, we should ensure that $X_1,\ldots,X_d$ are drawn uniformly from $\Fq^{(n-k)\times r}$ and that $A$ is also a uniform matrix.
Similarly to Lemma \ref{lm:SyndromeUniform} it can be proven that $X_1,\ldots,X_d$ 
follow uniform distribution over $\Fq^{(n-k)\times r}$ when certain conditions on $H$ and $\calE$ are satisfied. Experimental results show that $X_1,\cdots, X_d$ behave as uniformly distributed 
even when the conditions in Lemma \ref{lm:SyndromeUniform} are not met.
% While it is possible to give similar condition to Lemma \ref{lm:SyndromeUniform} for the case $d>2$, only the first $r$ rows of $A \in \Fq^{r(d-1) \times r(d-1)}$ can be considered as uniformly drawn but the remaining $(r-1)(d-1)$ are fixed.
% Even though $A$ is not uniform, 
Although $A$ cannot be considered to follow uniform distribution, experimental results show that the pairs $Z^{(1)}, A$ span the whole space $\Fq^{r(d-1)}$ with the same probability as given in Corollary \ref{cor:Pr(C_k^u)}.
With the assumption that the pairs $Z^{(1)}, A$ behave like uniformly random distributed with respect to Corollary \ref{cor:Pr(C_k^u)},
we can give a generalized version of Proposition \ref{prop:1}

\begin{proposition}\label{prop:2}
Let $\calC \subseteq \Fqm^n $ be an LRPC code having one 
    parity check matrix $H\in \Fqm^{(n-k)\times n}$ of support $\Span{\Fq}{H} = \calV_{\alpha, d}$ for some $\alpha \in \Fqm$ and a small integer $d\geq 2$. 
    Suppose $\be\in\Fqm^n$ is an error of rank $r$ and denote $\calE=\Span{\Fq}{\be}$
    and $\calS=\Span{\Fq}{\bs}$, where $\bs= \be H^\intercal$. Then, 
    the probability that 
    $\calV_{\alpha, r-1}.\calS = \calV_{\alpha, d+r-2}.\calE$ 
    is given by $1-\frac{q+1}{q-1} q^{-u}$, where $u=(n-k)-r$. 
\end{proposition}

% To successfully correct an error $\be$ of rank $r$, the syndrome equation $H\be^\intercal = \bs^\intercal$ should satisfy $(n-k)dr \geq nr$, indicating $R\leq 1 - \frac{1}{d}$. 
% By properly choosing $u$, we obtain the following main theorem.
% \begin{theorem}\label{th:d2rate}
%     Let $\calC \subseteq \Fqm^n $ be an LRPC code having one 
%     parity check matrice $H\in \Fqm^{(n-k)\times n}$ of support $\Span{\Fq}{H} = \calV$ for some $\alpha \in \Fqm$ and a small integer $d\geq 2$. 
%     For sufficiently large $m$, $n$ and $\delta \in (0,1)$,
%     when $u\geq n(\frac{1}{d}-\delta)$,
%     an error $\be\in\Fqm^n$ of rank $r=\delta n$ can be corrected with a failure rate in the order of $\frac{q^{-(u+1)}}{q-1}$ for a code rate 
%     $$
%     R = 1 - \delta - \frac{u}{n}.
%     $$
% \end{theorem}

==> parts/SuccesfulExpansion_1.tex <==
\textsl{% !TeX root = ../main.tex
\section{Successful subspace expansion.}\label{sec:Successful}
% In the previous section, we saw how it is possible to  increase the rate of some LRPC codes, while maintaining the same error correction capability.
% This is achieved thanks to an expansion that involves both the support of the syndrome and the product space where it is contained.


For BD-LRPC codes, assume $\calS \subseteq \Fqm$ is the subspace generated by the syndrome $\bs=\be H^\intercal$ and $\calV_{\alpha,d}.\calE \subseteq \Fqm$ is the product space between the parity-check matrix support $\calV_{\alpha,d}$ and the error support $\calE.$
In the previous section, we briefly pointed out that we can 
expand $\calS$ and $\calV_{\alpha,d}.\calE$ by 
 the product with $\calV_{\alpha,t}$, for a certain integer $t\geq 1$, 
 which leads to 
 $\calV_{\alpha,t}.\calS = \calV_{\alpha,d + t -1}.\calE$ with a high probability.
 In this section, we shall intensively discuss the probability of such a successful expansion.
 
Consider the space $\calE = \Span{\Fq}{\be}$ with a basis ${\bm\varepsilon} = (\varepsilon_1, \ldots, \varepsilon_r)$ and
$\calS =\Span{\Fq}{\bs}$, where $\bs=(s_1,\dots, s_{n-k})$ is the syndrome. Since $\calS$ is a subspace of the product space $\calV_{\alpha,d}.\calE$, we have
$$
   \calS \subseteq \calV_{\alpha,d}.\calE = \calE + \alpha \calE  + \ldots + \alpha^{d-1} \calE .   
$$
Thus  each $s_i \in \calS$ can be written as $s_i = \sum_{j=1}^d x_{i,j}\alpha^{j-1}$, where $x_{i,j}\in \calE$ for $j=1,\dots, d$.
Denote by $\ba_d$ the vector $\ba_d = (1,\alpha, \ldots, \alpha^{d-1})$, which is a basis of $\calV_{\alpha, d}$ \cc when $\dim(\calV_{\alpha, d}) =d$\cn.  Then we have $s_i = (x_{i,1}, \ldots, x_{i,d}) \ba_d^\intercal.$
Consider the matrix $X \in \calE^{(n-k) \times d}$ whose $i$-th row is given by $(x_{i,1}, \ldots, x_{i,d})$, where $1\leq i\leq n-k$. This gives 
$$
    \bs^\intercal
    =
    X \ba_d^\intercal = \bx_1^{\intercal} + \alpha \bx_2^{\intercal} + \dots + \alpha^{d-1} \bx_d^{\intercal},
$$ where
 $\bx_j^\intercal=(x_{1,j}, \dots, x_{n-k,j})\cc^\intercal \cn \in \calE^{n-k}$ denotes the $j$-th column of $X$.
We can expand each column $\bx_j^\intercal$ to the matrix $X_j \in \Fq^{(n-k) \times r}$ such that 
$
    X_j \bee^{\intercal} = \bx_j^\intercal.
$
The syndrome $\bs$ can then be obtained as 
\begin{equation}\label{eq:SyndromeSum}
    \bs^\intercal
    =
    X_1 \bee^\intercal + \alpha X_2 \bee^\intercal + \ldots + \alpha^{d-1} X_{d} \bee^\intercal. 
\end{equation}
\cc The vector $
    \ba_d \otimes \bee = 
    (\bee, \alpha \bee, \ldots, \alpha^{d-1} \bee) \in \Fqm^{dr},
$ is always a generator of $\calV_{\alpha,d}.\calE$
 implying
$\calV_{\alpha,d}.\calE = \Span{\Fq}{\ba_d \otimes \bee}.$ 
When $\dim(\calV_{\alpha,d}.\calE) = rd,$ the vector $\ba_d \otimes \bee$ is also a basis. \cn Using these notations we have 
\begin{equation}\label{eq:SyndromeAsMatrix}
    \bs^\intercal
    =
    \begin{pmatrix}
        X_1,  \ldots,  X_d 
    \end{pmatrix}
    (\ba_d \otimes \bee)^\intercal.
\end{equation}
This equation describes the coordinates of the syndrome with respect to the generator $\ba_d \otimes \bee$ of $\calV_{\alpha,d}.\calE$.
\cc
When $\dim(\calS) = \dim(\calV_{\alpha,d}.\calE) = dr$, 
the matrix $(X_1,\ldots, X_d)$ induces a one-to-one correspondence between $\bs$ and $\ba_d \otimes \bee$, thus $\bee$ can be uniquely determined.
\cn

\cc
\begin{remark}
    All the discussion above can be applied in the same way for a generic LRPC code.
    Let $H \in \Fqm^{(n-k)\times n}$ be a parity-check matrix such that $ \calH = \Span{\Fq}{H} = \Span{\Fq}{h_1, \ldots h_d}.$
    If we consider the ordered basis $\mathbf{h}_d = (h_1, \ldots h_d)$ for the support of $H$ and $\bee = (\varepsilon_1, \ldots, \varepsilon_r)$ an ordered basis of the support of the error, we can represent the syndrome $\bs = \be H^\intercal$ as a matrix over the basis $(\bb_d \otimes \bee)$ like we did in (\ref{eq:SyndromeAsMatrix}), i.e.
    $$
        \bs^{\intercal}=
    \begin{pmatrix}
        X_1,  \ldots,  X_d 
    \end{pmatrix}
    (\mathbf{h}_d \otimes \bee)^\intercal.
    $$
    Similarly, the components of the vector $(\mathbf{h}_d \otimes \bee)$ are a generator of the product space $\calH.\calE$ and , when the product space has dimension $dr$, the vector $(\mathbf{h}_d \otimes \bee)$ constitutes an ordered basis of $\calH.\calE.$
    
\end{remark}
\cn

Consider the cases where $\calS \subsetneq \calV_{\alpha,d}.\calE$ and start with the first expansion.
The expansion is given by $\calV_{\alpha,2} \calS = \calS + \alpha \calS \subseteq \calV_{\alpha,d+1}.\calE.$
Note that, since $\calS$ is the support of $s$, the support of $\alpha s$ is $\alpha \calS.$
As in (\ref{eq:SyndromeSum}), we can express $\alpha \bs$ as
\begin{equation*}\label{eq:AlphaSyndromeSum}
   \alpha \bs^\intercal 
%   \begin{pmatrix}
%        s_1 \\ \vdots \\ s_{n-k}
%    \end{pmatrix}
    =
    \alpha X_1 \bee^\intercal + \alpha^2 X_2 \bee^\intercal + \ldots + \alpha^d X_d \bee^\intercal 
\end{equation*}
Denote $\ba_{d+1} = (1,\alpha, \ldots, \alpha^{d})$. Then, \cc if $\dim(\calV_{\alpha,d+1}.\calE) = r(d+1)$, \cn
 a basis of $\calV_{\alpha,d+1}.\calE$ can be given by $\ba_{d+1} \otimes \bee = (\ba_d \otimes \bee, \alpha^d \bee) \in \Fqm^{(d+1)r}.$
Thus we have
\begin{equation}\label{eq:AlphaSyndromeAsMatrix}
    \alpha \bs^\intercal
    =
    \begin{pmatrix}
        \bzero & X_1 & \ldots & X_d 
    \end{pmatrix}
    (\ba_{d+1} \otimes \bee)^\intercal.
\end{equation}
Combining (\ref{eq:SyndromeAsMatrix}) and (\ref{eq:AlphaSyndromeAsMatrix}) gives the system
\begin{equation}\label{eq:Exp2AsMatrix}
    \begin{pmatrix}
        \bs^\intercal \\
        \alpha \bs^\intercal
    \end{pmatrix}
    =
    \begin{pmatrix}
        X_1 & X_2 & \ldots & X_d & \bzero \\
        \bzero & X_1 & X_2 & \ldots & X_d 
    \end{pmatrix}
    (\ba_{d+1} \otimes \bee)^\intercal.
\end{equation}
We can similarly extend \eqref{eq:Exp2AsMatrix}  for the general expansion $\calV_{\alpha,t}. \calS = \calV_{\alpha,d+t-1}.\calE.$
In this case $\ba_{d+t} \otimes \bee$ is a basis of $\calV_{d+t-1}.\calE$ and the coordinates of $(\ba_t \otimes \bs)^\intercal = (\bs, \alpha \bs, \ldots \alpha^{t-1} \bs)^\intercal$ can be expressed as
\begin{equation} \label{eq:ExpAsMatrix}
    \begin{pmatrix}
       \bs^\intercal \\ \alpha \bs^\intercal \\ \vdots \\ \alpha^{t-1} \bs^\intercal
    \end{pmatrix}
    =
    \begin{pmatrix}
        X_1 & X_2 & \cdots & X_d     & 0   & \cdots & 0 \\
        0   & X_1 & X_2 & \cdots & X_d & \cdots & 0 \\
        \vdots   &  & \ddots & \ddots  &  & \ddots & \vdots \\
        0   & \cdots &  0 & X_1  & X_2 & \cdots & X_d 
    \end{pmatrix}
    \begin{pmatrix}
        \bee^\intercal \\ \alpha \bee^\intercal \\ \vdots \\ \alpha^{d+t-2} \bee^\intercal 
    \end{pmatrix}.
\end{equation}
The above expansion is considered successful when
$\calV_{\alpha,t}. \calS = \calV_{\alpha, d+t-1}.\calE$, which
can be stated in terms of bases as $$\Span{\Fq}{\ba_t \otimes \bs} = \Span{\Fq}{\ba_{d+t-1} \otimes \bee}.$$
In order to ensure that the above equality holds, we need to consider the big matrix in (\ref{eq:ExpAsMatrix}).
Let $M_t$ be the $(n-k)t \times (d+t-1)r$ matrix on the right hand side of (\ref{eq:ExpAsMatrix}).
If $M_t$ has full rank $(d+t-1)r$, then there will be an invertible square sub-matrix $\hat{M_t}$ of order $(d+t-1)r$ in $M_t$ and a corresponding sub-vector $\hat{\bs} \in \Fqm^{(d+t-1)r}$ such that $\hat{\bs}^\intercal = \hat{M_t} (\ba_{d+t-1} \otimes \bee)^\intercal.$
This implies 
\begin{equation}\label{eq:se}
    \hat{M_t}^{-1}\hat{\bs}^\intercal  =  (\ba_{d+t-1} \otimes \bee)^\intercal.
\end{equation}
That is to say, all the entries of $(\ba_{d+t-1} \otimes \bee)$ can be obtained as $\Fq$-linear combinations of entries in $\hat{\bs}.$
In this case, we have that $\Span{\Fq}{\ba_{d+t-1} \otimes \bee} \subseteq \Span{\Fq}{\hat{\bs}}$ 
while $\Span{\Fq}{\hat{\bs}} \subseteq \Span{\Fq}{\ba_t\otimes\bs},$
from which $\Span{\Fq}{\ba_{d+t-1} \otimes \bee} = \Span{\Fq}{\ba_t\otimes\bs}.$ Therefore, 
the successful expansion $\calV_{\alpha,t} \calS = \calV_{\alpha,d+t-1}.\calE$ can be achieved if and only if $M_t$ has full rank $(d+t-1)r$, which is only possible when $(n-k)t\geq (d+t-1)r$.
\color{black}
% The entries of the matrices $X_i \in \Fq^{(n-k)\times r}$ in (\ref{eq:ExpAsMatrix}) depend on the syndrome $\bs.$ 
% Heuristically these matrices behave as random matrices uniformly drawn from $\Fq^{(n-k)\times r}$.
% We shall use this assumption and establish a necessary and sufficient condition for the matrix $M_t$ to have full rank $(d+t-1)r.$
% The assumption that $X_i$ follows uniform distribution over $\Fq^{(n-k)\times r}$ can be justified under certain conditions on $H$, which is discussed in Lemma \ref{lm:SyndromeUniform}.
Observe that one necessary (but not sufficient) condition for $M_t$ to be of full rank $(d+t-1)r$ is $\Rank(X_1) = \Rank(X_d) = r.$ Below we shall investigate the necessary and sufficient 
condition for $\Rank(M_t) = (d+t-1)r$.


\iffalse
The derivation of a necessary and sufficient condition is relatively complicated for general $d$.

Denote $u = n-k-r$. Then we have $u \geq \frac{r}{t}(d-1).$
In the following, we will show that the probability that $M_t$ has full rank $(d+t+1)r$ for $t = r-1$, is in the order of $1 - q^{-u + 1}.$
% \begin{theorem}\label{th:d2rate}
%     Let $\calC \subseteq \Fqm^n $ be an LRPC code of density $2$. That is an LRPC code that admits a parity-check matrices $H$ of support $\Span{\Fq}{H} = \Span{\Fq}{1,\alpha}$ for some $\alpha \in \Fqm.$ 
%     Let $R$ be the rate of $\calC$ and let $\delta$ be the error rate.
%     Provided that $m$ and $n$ are sufficiently large, it is possible to correct an error of rank $\delta n$ with failure rate in the order of $q^{-u}$ with a rate
%     $$
%         R \leq 1 - \delta - u/n.
%     $$
% \end{theorem}

From \eqref{eq:ExpAsMatrix} the matrix $M_t$ for $d=2$ is given by
\begin{equation}\label{eq:Mt2}
    M_t 
    =
    \begin{pmatrix}
        X_1 & X_2 &        &        &       \\
            & X_1 & X_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & X_1    & X_2   
    \end{pmatrix}
    \in \Fq^{(r+u)t \times (t+1)r}.
\end{equation}
% Each of the matrices $X_1, X_2 \in \Fq^{(r+u)\times r}$ will be of full rank $r$ with probability $\prod_{i= 0}^{r-1} (q^{r+u} - q^i)/q^{r(r + u)} \approx 1 - q^{(r-1)(r+u)}(q^r-1)/(q-1) q^{-r(r+u)} \approx 1 - q^{-u}.$
% These conditions are unfortunately not enough to guarantee that $M_t$ is of full rank.
Suppose that $X_1,X_2$ are of full rank $r$, we can analyze the problem as follows.
Firstly, choose a permutation matrix $P_0$ such that 
$P_0(X_1,X_2) = \begin{psmallmatrix} Y_1 & Y_2\\ Z_1 & Z_2 \end{psmallmatrix}$,
where $Y_1 \in \Fq^{r \times r}$ is an invertible matrix and $Z_1, Z_2 \in \Fq^{u \times r}.$ 
Iteratively applying $P_0$ on $X_1, X_2$ in $M_t$, we obtain
\begin{equation}\label{eq:Mt2_stairs}
M_t\rightarrow    P M_t 
    =
    \begin{pmatrix}
        Y_1 & Y_2 &        &        &       \\
            & Y_1 & Y_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & Y_1    & Y_2   \\
        Z_1 & Z_2 &        &        &       \\
            & Z_1 & Z_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & Z_1    & Z_2      
    \end{pmatrix}
    \in \Fq^{(r+u)t \times (t+1)r}.
\end{equation}
It is clear that $M_t$ has full rank if and only if $PM_t$ has full rank.
% In particular, since $X_1$ is of full rank $r$, there exists a permutation $P$ such that $Y_1 \in \Fq^{r \times r}$ is invertible and $Z_1 \in \Fq^{u \times r}.$
% The same permutation will split $X_2$ into $Y_2 \in \Fq^{r\times r}$ and $Z_2 \in \Fq^{u \times r}.$
Since $Y_1$ is invertible, there exists a matrix $A \in \Fq^{r \times r}$ such that $Y_1 A = -Y_2$. Moreover, we have $\RowSpan(A) = \RowSpan(Y_2).$
We can use this relation to further transform $M_t$ as follows
\begin{equation}
M_t\rightarrow PM_t=\begin{pmatrix}
        Y_1 & Y_2 &        &        &       \\
            & Y_1 & Y_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & Y_1    & Y_2   \\
        Z_1 & Z_2 &        &        &       \\
            & Z_1 & Z_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & Z_1    & Z_2      
    \end{pmatrix} \rightarrow
    \begin{pmatrix}
        Y_1 &     &        &        &       \\
            & Y_1 & Y_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & Y_1    & Y_2   \\
            & Z   &        &        &       \\
            & Z_1 & Z_2    &        &       \\
            &     & \ddots & \ddots &       \\
            &     &        & Z_1    & Z_2      
    \end{pmatrix},
\end{equation}
where $Z = Z_1 A + Z_2.$
By iteratively applying this reduction $t$ times to eliminate all the instances of $Y_2$,
we have the following elementary transformations on $M_t$:
\begin{equation}\label{eq:redMt2}
M_t \rightarrow PM_t \rightarrow    \Tilde{M_t}
    = 
    \begin{pmatrix}
        Y_1 &     &        &        &           \\
            & Y_1 &        &        &           \\
            &     & \ddots &        &           \\
            &     &        & Y_1    &           \\
            % &     &        &        & ZA^{t-1}  \\
            % &     &        &        & ZA^{t-2}  \\
            % &     &        &        & \vdots    \\
            &     &        &        & \Tilde{Z}     
    \end{pmatrix} \text{ with } \Tilde{Z}=\begin{pmatrix}
    ZA^{t-1} \\ ZA^{t-2} \\ \vdots \\ Z
    \end{pmatrix}.
\end{equation}
% Denote by $\Tilde{Z}  
% $the lower part of $\Tilde{M}_t$ formed by $Z, ZA, \dots, ZA^{t-1}$.
It is readily seen that 
$$
    \Rank(M_t) =\Rank(\Tilde{M_t}) = t \Rank(Y_1) + \Rank(\Tilde{Z}) = tr + \Rank(\Tilde{Z}).
$$
Hence the probability of $\Rank(M_t)= (t+1)r$ is the same as the probability probability that 
$\RowSpan(\Tilde{Z}) = \Fq^r$ and $\Rank(Y_1) = r$.
From the definition of $\Tilde{Z}$, we have 
$$\RowSpan(\Tilde{Z}) = \RowSpan(Z) + \ldots + \RowSpan(ZA^{t-1}) = \Fq^r.$$
Calculating this probability requires a detailed investigation of the relation between rows in the $\RowSpan(ZA^i)$ for $i=0,1,\dots,t-1$. 
Section \ref{sec:ExpRowSub} is dedicated to the calculation of this probability for uniformly distributed $Z$ and $A$.

Recall that $X_1, X_2$ are obtained from the syndrome $\bs$ over $\calE$.
Heuristically $X_1, X_2$ follow a uniform distribution over $\Fq^{(n-k)\times r}$.
This property is theoretically confirmed in the following lemma.
\begin{lemma}\label{lm:SyndromeUniform}
Let the $(n-k)\times n$ matrix $H$ over $\calV_{\alpha,2}$
be decomposed as $H = H_1 + \alpha H_2,$ where $H_1,H_2 \in \Fq^{(n-k) \times n}.$
Let $\calE\subseteq \Fqm$ be an $\Fq$-linear subspace of dimension $r$ such that $\dim(\calV_{\alpha, 2}.\calE) = 2r$.
    If $\Rank \begin{psmallmatrix} H_1 \\ H_2 \end{psmallmatrix} = 2(n-k)$ then, for each $\bs \in (\calV_{\alpha, 2}.\calE)^{n-k}$ the set 
    $$
        \Sol(\bs)=\{\be \in \calE^n \mid H \be^\intercal = \bs^\intercal \}
    $$ 
    has the same cardinality $q^{r(2k-n)}$.
\end{lemma}
\begin{proof}
    If the subspace $\calV_{\alpha,2}.\calE=\Span{\Fq}{1, \alpha}.\calE$ has dimension $2r$, it can be decomposed into the direct sum of $\calE$ and $\alpha \calE.$
    Then the vector $\bs$ can be decomposed into $\bs = \bs_1 + \alpha \bs_2$ where $\bs_1,\bs_2 \in \calE.$
    If there exists $\be \in \calE^n$ such that $H \be^\intercal = \bs^\intercal$, then $H_1 \be^\intercal = \bs_1$ and $H_2 \be^\intercal = \bs_2$.
    We can expand $\bs_1^{\intercal}, \bs_2^\intercal$ into two matrices $X_1, X_2 \in \Fq^{(n-k)\times r}$ such that
    $$
        \bs_1^\intercal = X_1 \begin{pmatrix} \varepsilon_1 \\ \vdots \\ \varepsilon_r \end{pmatrix}, \quad \bs_2^\intercal = X_2 \begin{pmatrix} \varepsilon_1 \\ \vdots \\ \varepsilon_r \end{pmatrix}. 
    $$
    Similarly we can expand $\be^\intercal \in \calE^n$ to a matrix $E \in \Fq^{n \times r}$ such that $\be^\intercal = E (\varepsilon_1, \ldots, \varepsilon_r)^\intercal.$
    We obtain the expanded system 
    \begin{equation}\label{eq:SyndromeUniformExpanded}
        \begin{pmatrix}
            H_1 \\
            H_2
        \end{pmatrix}
        E 
        =
        \begin{pmatrix}
            X_1 \\
            X_2
        \end{pmatrix}
    \end{equation}
    By hypothesis $H' = \begin{psmallmatrix} H_1 \\ H_2 \end{psmallmatrix}$ has rank $2(n-k).$
    Restrict the system (\ref{eq:SyndromeUniformExpanded}) to the $i$-th column of $\begin{psmallmatrix} X_1 \\ X_2 \end{psmallmatrix}$ there are possible $q^{2k - n}$ choices of the $i$-th column of $E$ that will be a solution of the restricted system.
    For each choice of  $\begin{psmallmatrix} X_1 \\ X_2 \end{psmallmatrix}$ there will be $q^{r(2k - n)}$ possible matrices $E$ that satisfy (\ref{eq:SyndromeUniformExpanded}). 
    This is equivalent to say that, for each $\bs \in (\calV_{\alpha, 2}.\calE)^{n-k}$, the set $\Sol(\bs)$ has $q^{r(2k - n)}$ elements.
    % \qed
\end{proof}

From Lemma \ref{lm:SyndromeUniform} one can clearly see that, when $\be$ is uniformly drawn from
$\calE^n$, if $\dim(\calV_{\alpha,2}.\calE) = 2r$,  the matrices $X_1,X_2$ derived from $\bs=\bs_1+\alpha \bs_2$ follow a uniform distribution. Note that the matrix $Z=Z_1A+Z_2$ and $A$  can be deemed to follow a uniform distribution 
over $\Fq$. As a matter of fact, assume $X_2$ in (\ref{eq:Mt2}) is
uniformly drawn from $\Fq^{(n-k) \times r}$. Recall that $\begin{psmallmatrix}
Y_2 \\ Z_2
    \end{psmallmatrix}
    =P_0X_2
    $
    and
$A = -Y_1^{-1} Y_2$. Thus we have
\begin{equation}\label{eq:AZ_uniform}
\begin{pmatrix}
        A \\ Z
    \end{pmatrix} 
    =
    \begin{pmatrix}
        -Y_1^{-1} & \bzero \\
        - Z_1 Y_1^{-1} & I_{u}
    \end{pmatrix}
    \begin{pmatrix}
        Y_2 \\ Z_2
    \end{pmatrix}
    = \begin{pmatrix}
        -Y_1^{-1} & \bzero \\
        - Z_1 Y_1^{-1} & I_{u}
    \end{pmatrix}
    P_0X_2
\end{equation} 
It is readily seen that 
$\begin{psmallmatrix}  A \\ Z \end{psmallmatrix}$ 
has a one-to-one correspondence to the uniformly distributed $X_2$. Therefore,  $\begin{psmallmatrix}  A \\ Z \end{psmallmatrix}$  also follows a uniform distribution.

\smallskip

As it will be shown in Corollary \ref{cor:Pr(C_k^u)} in Section \ref{sec:ExpRowSub}, the probability that a matrix $\begin{psmallmatrix}  A \\ Z \end{psmallmatrix}$ uniformly drawn from $\Fq^{(r+u) \times r}$ leads to $\sum_{i=0}^{r-1} \RowSpan(ZA^{i}) = \Fq^r$ is in the order of $1 - \frac{q^{-u+1}}{q-1}.$ 
At the same time, the probability that a random matrix $X_1$, uniformly chosen in $\Fq^{(r+u)\times r}$, has rank $r$ is given by 
$$
    q^{-(r+u)r}\prod_{i = 0}^{r-1}(q^{r+u} - q^i) \approx 1 - q^{-r-u} \sum_{i=0}^{r-1}q^i  \approx 1 - \frac{q^{-u}}{(q-1)}.
$$
Combining the above analysis, we have the following result:

\begin{proposition}\label{prop:1}
Let $\calC \subseteq \Fqm^n $ be an LRPC code having one 
    parity-check matrix $H\in \Fqm^{(n-k)\times n}$ of support $\Span{\Fq}{H} = \calV_{\alpha, 2}$ for some $\alpha \in \Fqm.$ 
    Suppose $\be\in\Fqm^n$ is an error of rank $r$ and denote $\calE=\Span{\Fq}{\be}$
    and $\calS=\Span{\Fq}{\bs}$, where $\bs= \be H^\intercal$. Then, 
    the probability that 
    $\calV_{\alpha, r-1}.\calS = \calV_{\alpha, r}.\calE$ 
    is given by $1- \frac{q+1}{q-1} q^{-u}$, where $u=(n-k)-r$. 
\end{proposition}




% obtain that for an LRPC code $\calC$
% with parity-check matrix $H\in \Fqm^{(n-k)\times n}$ having support $\Span{\Fq}{H} = \Span{\Fq}{1,\alpha}$ and an error $\be$ of rank $r$ uniformly drawn from $\calE^n$, 
% under the condition that $(n-k)\geq r + \frac{r}{r-1}$,
% the probability that the syndrome space $\calS$ satisfying 
% $\calV_{\alpha, r-1}.\calS = \calV_{\alpha, r}. \calE$ is in the order of $\frac{q^{-u+1}}{q-1}$.



% \begin{theorem}\label{th:d2rate}
%     Let $\calC \subseteq \Fqm^n $ be an LRPC code having one 
%     parity-check matrice $H\in \Fqm^{(n-k)\times n}$ of support $\Span{\Fq}{H} = \Span{\Fq}{1,\alpha}$ for some $\alpha \in \Fqm.$ 
%     For sufficiently large $m$, $n$ and $k< \frac{n}{2}$,
%     an error $\be\in\Fqm^n$ of rank $r\leq \frac{n}{2}$ can be corrected with a failure rate in the order of $\frac{q^{-(u+1)}}{q-1}$, where $u=(n-k)-r$.
% \end{theorem}

% It is now time to give a good reason why $X_1, X_2$ in (\ref{eq:Mt2}) can be considered as independently drawn from a uniform distribution.

% When the conditions of this lemma are satisfied, the matrices in (\ref{eq:Mt2}) can be considered uniformly chosen and independent.
% For these codes we can then rigorously prove that Theorem \ref{th:d2rate}.
% For the other cases it seems fair to assume that the matrices $X_1,X_2$ will still behave like if they were independently uniformly drawn.

% \subsubsection{Consecutive power LRPC codes}
We can now extend our analysis for a general small integer $d$.
A successful expansion is obtained when there exists $t$ such that $\calV_{\alpha,t}.\calS = \calV_{\alpha,d+t-1}.\calE.$
Let $\bee \in \Fqm^{r}$ be a basis of the error support $\calE$ and let $\bs \in \Fqm^{n-k}$ be a basis of the syndrome support.
If we define $\ba_t = (1, \alpha, \ldots, \alpha^{t-1})$, we have that $\calV_{\alpha,t}.\calS = \Span{\Fq}{\ba_t \otimes \bs}$ and $\calV_{\alpha, d+t-1} = \Span{\Fq}{\ba_{d+t-1} \otimes \bee}.$
The syndrome expansion was already modeled in (\ref{eq:ExpAsMatrix}) giving the equation $(\ba_t \otimes \bs)^\intercal = M_t(\ba_{d+t-1} \otimes \bee)^\intercal $ where 
\begin{equation} \label{eq:Mtd}
    M_t
    =
    \begin{pmatrix}
        X_1 & X_2 & \cdots & X_d       &     &        &     \\
            & X_1 & X_2    & \cdots    & X_d &        &     \\
            &     & \ddots & \ddots    &     & \ddots &     \\
            &     &        & X_1       & X_2 & \cdots & X_d 
    \end{pmatrix}.
\end{equation}

In (\ref{eq:ExpAsMatrix}), when $\Rank(M_t) = (d+t-1)r$, each component of $\ba_{d+t-1} \otimes \bee$ can be expressed as an $\Fq$-linear combination of components of $\ba_t \otimes \bs,$ indicating  $\calV_{\alpha,t}.\calS = \calV_{\alpha,d+t-1}.\calE.$
\fi

\smallskip

Assume $\Rank(X_1) = r$. We can rearrange the rows of $X_1$ such that $X_1 \rightarrow \begin{psmallmatrix}
Y_1 \\ Z_1
\end{psmallmatrix}$ with $\Rank(Y_1)=r$. Furthermore, we can rearrange the rows of $M_t$ to obtain  the matrix
\begin{equation}\label{eq:Mtd_stairs}
    P M_t
    =
    \begin{pmatrix}
        Y_1 & Y_2 & \cdots & Y_d       &     &        &     \\
            & Y_1 & Y_2    & \cdots    & Y_d &        &     \\
            &     & \ddots & \ddots    &     & \ddots &     \\
            &     &        & Y_1       & Y_2 & \cdots & Y_d \\
        Z_1 & Z_2 & \cdots & Z_d       &     &        &     \\
            & Z_1 & Z_2    & \cdots    & Z_d &        &     \\
            &     & \ddots & \ddots    &     & \ddots &     \\
            &     &        & Z_1       & Z_2 & \cdots & Z_d 
    \end{pmatrix},
\end{equation}
where $Y_i \in \Fq^{r\times r}$, $Z_i \in \Fq^{u \times r}$ \cc where $u=n-k-r$ \cn and $\Rank(Y_1)=r$.
Since $Y_1$ is invertible, there exist square matrices  $A_1, \ldots, A_{d-1}$ such that $Y_1 A_{i} = -Y_{i+1}$ for $i=1, \dots, d-1$.
\cc Using the matrices $A_i$ for $1\leq i<d$ and elementary rows and columns operations\cn,
we can transform $PM_t$ to
\begin{equation}\label{eq:Mtd_1}
    M_t^{(1)}
    =
    \begin{pmatrix}
        Y_1 &     	\bzero	&    \cdots    &     \bzero      	 &     &        &     \\
            & Y_1 		& Y_2    & \cdots    	 & Y_d &        &     \\
            &     		& \ddots & \ddots    	 &     & \ddots &     \\
            &     		&        & Y_1       	 & Y_2 & \cdots & Y_d \\
            & Z_1^{(1)} & \cdots & Z_{d-1}^{(1)} &     &        &     \\
            & Z_1 		& Z_2    & \cdots    	 & Z_d &        &     \\
            &     		& \ddots & \ddots    	 &     & \ddots &     \\
            &     		&        & Z_1       	 & Z_2 & \cdots & Z_d 
    \end{pmatrix},
\end{equation}
where $Z_{i}^{(1)} = Z_1 A_i + Z_{i+1}.$
We can continue reducing the second block with the same matrices $A_1, \ldots, A_{d-1}$.
This will give us the further reduction
\begin{equation}\label{eq:Mtd_2}
    M_t^{(2)}
    =
    \begin{pmatrix}
        Y_1 &    \bzero &        \cdots		&    \bzero    &     			 &         &     \\
            & Y_1 &      \bzero  		&    \cdots    &    \bzero 			 &         &     \\
            &     & \ddots      & \ddots   &     & \ddots &     \\
            &     &        		& Y_1    & Y_2 			 & \cdots  & Y_d \\
            &     & Z_1^{(2)} 	& \cdots & Z_{d-1}^{(2)} &     	   &     \\
            &     & Z_1^{(1)}   & \cdots & Z_{d-1}^{(1)} &         &     \\
            &     & \ddots 		& \ddots &     			 & \ddots  &     \\
            &     &        		& Z_1    & Z_2 			 & \cdots  & Z_d 
    \end{pmatrix},
\end{equation}
where $Z_{i}^{(2)} = Z_1^{(1)} A_i + Z_{i+1}^{(1)}$ for $1\leq i<d$ and $Z_{d}^{(1)} = \bzero.$
Let us define $Z^{(j)} \in \Fq^{u \times (d-1)r}$ as $Z^{(j)} = ( Z_1^{(j)}, \cdots, Z_{d-1}^{(j)})$ and the square matrix $A \in \Fq^{(d-1)r \times (d-1)r}$ as
\begin{equation}\label{eq:matrix_A}
    A =
	\begin{pmatrix}
		A_1 & A_2 & \cdots & A_{d-2} & A_{d-1} 	\\
		I_r &     &        &         &  \bzero  \\
			& I_r &  	   &         &  \bzero  \\
			&	  & \ddots &         &  \vdots  \\
			&     &		   & I_r     & 	\bzero	
		\end{pmatrix}.
\end{equation}
Observe that $$Z^{(2)} = ( Z_1^{(2)} \cdots Z_{d-1}^{(2)})= ( Z_1^{(1)}, \cdots, Z_{d-1}^{(1)}) A = Z^{(1)}A.$$ More generally,
we have $Z^{(j+1)} = Z^{(j)} A$, implying that 
$Z^{(j+1)} = Z^{(1)}A^j$ for $j=1, 2,\dots, t-2$. 
Therefore, after iterating the reduction step $t$ times, we obtain the matrix
\begin{equation}\label{eq:Mtd_t}
    M_t^{(t)}
    =
    \begin{pmatrix}
        Y_1 &     &        &     &     			  \\
            & Y_1 &        &     &     			  \\
            &     & \ddots &     &     			  \\
            &     &        & Y_1 &  			  \\
            &     &        &     & Z^{(1)}A^{t-1} \\
            &     &        &     & Z^{(1)}A^{t-2} \\
            &     &        &     & \vdots         \\
            &     &        &     & Z^{(1)} 		  
    \end{pmatrix}.
\end{equation}
Denote \begin{equation}\label{eq:MtZA}
M_t(Z^{(1)}, A) =   \begin{pmatrix}
Z^{(1)} \\ Z^{(1)} A \\ \vdots \\ Z^{(1)} A^{t-1}
\end{pmatrix}
\in \Fq^{ut \times r(d-1)}.
\end{equation}
From \eqref{eq:Mtd_t}
 we have
$$
    \Rank(M_t^{(t)}) = t \Rank(Y_1) + \Rank(M_t(Z^{(1)},A)) =  rt + \Rank(M_t(Z,A)).
$$
The operations we applied to get $M_t^{(t)}$ from $M_t$ are all linear and invertible, therefore $\Rank(M_t) = \Rank(M_t^{(t)})$.
This leads to the following result.
\cc
\begin{proposition}\label{prop:0}
	Let $M_t$ be the matrix in \eqref{eq:ExpAsMatrix} and  $M_t(Z^{(1)},A)$ be the matrix defined in \eqref{eq:MtZA}. If $\Rank(X_1)=r$ and  $\Rank(M_t(Z^{(1)},A)) = (d-1)r$ then the equality $\calV_{\alpha, t}.\calS = \calV_{\alpha, d+t-1}.\calE$ holds.
\end{proposition} 

Note that it is still possible that $\calV_{\alpha, t}.\calS = \calV_{\alpha, d+t-1}.\calE$ with $\dim(\calV_{\alpha, d+t-1}.\calE) < (d+t-1)r.$
In this case, in order to have a successful expansion, it will be sufficient that $\Rank(M_t) = \dim(\calV_{\alpha, d+t-1}.\calE).$
For the rest of this paper we will consider the worst case where $\dim(\calV_{\alpha, d+t-1}.\calE) = (d+t-1)r.$
This means we need to estimate the probability that $\Rank(M_t) = (d+t-1)r$ which, thanks to
Proposition \ref{prop:0}, can be transformed to establish the probability that $\Rank(X_1) = r$ and that $\Rank(M_t(Z^{(1)},A)) = (d-1)r.$
In our analysis, we will consider the matrices $X_1, \ldots, X_d$ as independently chosen from a uniform distribution.
This assumption is true for certain parameters as in the following lemma.
%Outside of these parameters we will use the heuristic that the matrices $X_1, \ldots, X_d$ behave like if they were independently chosen from a uniform distribution.
\cn

% In Section \ref{sec:ExpRowSub} we will investigate the probability of $\Rank(M_t(Z,A)) = (d+t-1)r$ for uniformly distributed matrices 
% \cc 
% $Z \in \Fq^{u\times r(d-1)}, A \in \Fq^{r(d-1)\times r(d-1)}.$
% \cn
% In the decoding procedure, it can actually be proven that $X_1,\ldots,X_d$ 
% follow uniform distribution over $\Fq^{(n-k)\times r}$ when certain conditions on $H$ and $\calE$ are satisfied.
\cred
In \cite[Renner, Theorem 11]{renner20} and later in \cite[Burle, Proposition 3]{Burle23}, in order to establish the probability that the syndrome support is equal to the product space.
In both works, it was proven that the syndrome can be considered as a vector whose entries are uniformly chosen from the product space.
For the sake of completeness we report here in our notation the results in \cite{Burle23} that show why we can consider $X_1, \ldots, X_d$ as matrices independently and uniformly chosen from $\Fq^{(n-k)\times r}$ 
\begin{lemma}\label{lm:SyndromeUniform}

\end{lemma}

\cn

\begin{lemma}\label{lm:SyndromeUniformOld}
Let the $(n-k)\times n$ matrix $H$ over $\calV_{\alpha,d}$
be decomposed as $H = H_1 + \cdots  + \alpha^{d-1} H_{d},$ where $H_1,\ldots, H_{d} \in \Fq^{(n-k) \times n}.$
Let $\calE\subseteq \Fqm$ be an $\Fq$-linear subspace of dimension $r$ such that $\dim(\calV_{\alpha, d}.\calE) = dr$.
    If $\Rank \begin{psmallmatrix} H_1 \\ \vdots \\ H_{d} \end{psmallmatrix} = d(n-k)$ \cc and $n \geq (n-k)d$\cn, then 
    the matrices $X_1, \dots, X_d$ in \eqref{eq:SyndromeSum} follow a uniform distribution over $\Fq^{(n-k)\times r}$.
%    for each $\bs \in (\calV_{\alpha, d}.\calE)^{n-k}$ the set 
%    $$
%        \Sol(\bs)=\{\be \in \calE^n \mid H \be^\intercal = \bs^\intercal \}
%    $$ 
%    has the same cardinality $q^{r(2k-n)}$.
\end{lemma}
\begin{proof}
    If the subspace $\calV_{\alpha,d}.\calE=\Span{\Fq}{1,\ldots, \alpha^{d-1}}.\calE$ has dimension $dr$, it can be decomposed into the direct sum of $\calE,\alpha \calE, \ldots,\alpha^{d-1} \calE.$
    Recall from \eqref{eq:SyndromeSum} that 
    a vector $\bs$ in $\calV_{\alpha,d}.\calE$ can be decomposed as 
    $$
     \bs^\intercal
    =
    X_1 \bee^\intercal + \alpha X_2 \bee^\intercal + \ldots + \alpha^{d-1} X_{d} \bee^\intercal. 
    $$
    Suppose  $\bs$ is a syndrome of an error $\be$, 
    we have 
    $$
    \bs^\intercal= H\be^\intercal = H_1\be^\intercal + \cdots  + \alpha^{d-1} H_{d}\be^\intercal. 
    $$
    We can expand $\be \in \calE^n$ to a matrix $E \in \Fq^{n \times r}$ such that $\be^\intercal = E (\varepsilon_1, \ldots, \varepsilon_r)^\intercal.$
    Then we obtain the expanded system 
    \begin{equation}\label{eq:SyndromeUniformExpanded}
        \begin{pmatrix}
            H_1 \\
            \vdots \\
            H_{d}
        \end{pmatrix}
        E 
        =
        \begin{pmatrix}
            X_1 \\
            \vdots \\
            X_{d}
        \end{pmatrix}.
    \end{equation}
    By hypothesis the matrix $ \begin{psmallmatrix} H_1 \\ \vdots \\ H_{d} \end{psmallmatrix}$ has rank $d(n-k).$
    If we restrict the system (\ref{eq:SyndromeUniformExpanded}) to the $i$-th column of $\begin{psmallmatrix} X_1 \\ \vdots \\X_{d} \end{psmallmatrix}$ there are possible $q^{n - (n-k)d}$ choices of the $i$-th column of $E$ that will be a solution of the restricted system.
    For each choice of  $\begin{psmallmatrix} X_1 \\ \vdots \\ X_{d} \end{psmallmatrix}$ there will be $\cc q^{r(n - (n-k)d) \cn}$ possible matrices $E$ that satisfy (\ref{eq:SyndromeUniformExpanded}). 
    This implies that the matrices $X_1, \dots, X_d$ follow the uniform distribution over $\Fq^{(n-k)\times r}$.
%    This is equivalent to saying that, for each $\bs \in (\calV_{\alpha, 2}.\calE)^{n-k}$, the set $\Sol(\bs)$ has $q^{r(dk - (d-1)n)}$ elements.
    % \qed
\end{proof}
\cc
Recall that the expanded system obtained from the syndrome has $rd(n-k)$ equations over $\Fq$ and $rd$ variables.
In order to have unique decoding it is needed that $rd(n-k) \geq nr$,
implying $n \leq d(n-k).$ Hence the condition $n \leq d(n-k)$ is critical for unique decoding. The equality corresponds to the case where the expanded linear system has exactly the same number of variables and equations.

When we consider the problem of error support recovery, we can find parameters for which the matrices $X_1, \ldots, X_d$ can be considered as independently chosen from a uniform distribution.
In the case of $n \leq d(n-k)$, we will use the heuristic that they will still behave as if they were independently chosen from a uniform distribution.
Notice that a similar assumption is used in the first step of the decoding algorithm of LRPC codes.
The probability that the syndrome generates the product space $\calE.\calH$ is calculated assuming that the components of the syndrome are independently chosen from a uniform distribution in $\calE.\calH.$
In particular, for a given vector $\bs \in (\calE.\calH)^{(n-k)},$ it is guaranteed that there exists an error of length $n$ with support in $\calE$ such that $\bs=\be H^\intercal$ only in the case where $nr \geq rd(n-k).$


% Experimental results indicate that $X_1,\cdots, X_d$ behave as uniformly distributed even when the conditions in Lemma \ref{lm:SyndromeUniform} are not met. Although $A$ defined in \eqref{eq:matrix_A} cannot be considered to follow a uniform distribution, experimental results show that the rows of the matrix $M_t(Z^{(1)}, A)$ span the whole space $\Fq^{r(d-1)}$ with the same probability as given in Corollary \ref{cor:Pr(C_k^u)}.


Now our task is to investigate the probability of $\Rank(M_t(Z,A)) = (d+t-1)r$ as characterized in Proposition \ref{prop:0}.
We below divide our discussion in two cases. For the case of $d=2$, the matrices $Z, A$ can be deemed 
as uniformly distributed, and the probability is analyzed in great detail in Section \ref{sec:ExpRowSub}; and for the cases that $d>2$,  we investigate the probability by both theoretic analysis and computational simulations.



\subsection{The case $d=2$}\label{subsec: d=2}
It is worth noting that, in the special case $d=2$, the matrix $\begin{psmallmatrix}
A \\ Z^{(1)} 
\end{psmallmatrix},$ can be considered as uniformly drawn in $\Fq^{(u+r) \times r}.$  
Indeed, for $d=2$, we have that $Z^{(1)} = Z_1 A_1 + Z_2$ while $Z^{(i)} = Z^{(1)} A_1^{i-1}$ and $A = A_1.$
Assuming that the matrices $X_1,X_2$ derived from $\bs=\bs_1+\alpha \bs_2$ follow a uniform distribution in $\Fq^{(r+u) \times r}$, the matrices $Z^{(1)}=Z_1A_1+Z_2 \in\Fq^{u \times r}$ and $A_1 \in \Fq^{r \times r}$  can be deemed to follow a uniform distribution. 
As a matter of fact, assume $X_1$ satisfies the necessary condition $\Rank(X_1) = r.$
By $\begin{psmallmatrix}
Y_2 \\ Z_2
\end{psmallmatrix}
=P_0X_2
$
and
$A = -Y_1^{-1} Y_2$, we have
\begin{equation}\label{eq:AZ_uniform}
\begin{pmatrix}
A \\ Z^{(1)}
\end{pmatrix} 
=
\begin{pmatrix}
-Y_1^{-1} & \bzero \\
- Z_1 Y_1^{-1} & I_{u}
\end{pmatrix}
\begin{pmatrix}
Y_2 \\ Z_2
\end{pmatrix}
= \begin{pmatrix}
-Y_1^{-1} & \bzero \\
- Z_1 Y_1^{-1} & I_{u}
\end{pmatrix}
P_0X_2.
\end{equation} 
It is readily seen that 
$\begin{psmallmatrix}  A \\ Z^{(1)} \end{psmallmatrix}$ 
has a one-to-one correspondence to the uniformly distributed $X_2$. Therefore,  $\begin{psmallmatrix}  A \\ Z^{(1)} \end{psmallmatrix}$  also follows a uniform distribution.

A complete description of the probability that the rows of $M_t(Z^{(1)},A)$ span the whole space $\Fq^r$ in the case $d=2$ will be done in Section \ref{sec:ExpRowSub}.
Since the case $d=2$ covers all the LRPC codes of density $2$ we consider this case as the most important.
For $d>2$ the family of BD-LRPC codes represent a small fraction of all the possible LRPC codes of density $d$, especially for large value of $d,$ moreover the minimal value of the parameter $m$ becomes quickly impractical as $d$ grows.

\subsection{The case where $d>2$ and $r=1$}\label{subsec:d>2}
In this case, the matrix $A$ in equation (\ref{eq:matrix_A}) becomes increasingly sparse as $d$ grows.
Consequently, the tools developed in Section \ref{sec:ExpRowSub} are not suitable to directly analyze this case. Nevertheless, we can provide a rigorous description for the sparsest case.

For simplicity of notation, within this section we denote $n = d-1$
We can consider the case $r=1$ for which $A'$ is in the form
$$
A' = \begin{pmatrix}
    a_{n-1} & a_{n-2} & \cdots & a_{1} & a_{0}\\
    1   & & & & 0\\
     & 1 &&& 0 \\
     && \ddots && \vdots \\
     &&& 1&0 \\
\end{pmatrix}.
$$
As we will see in Lemma \ref{lm:BasisChangeInv}, for any $Z  \in \Fq^{u \times n}$ we have that the dimension of the space generated by the rows of $Z, ZA, \ldots, ZA^{n-1}$ is the same as the dimension of the space generated by the rows of $ZB(B^{-1} A' B)^i$ whenever $B$ is invertible.
If $Z$ is drawn from a uniform distribution so it is for $ZB.$
Take $B$ the invertible matrix having $1$ on its anti-diagonal and zero elsewhere. Then the matrix 
\begin{equation}\label{eq:comp_mat}
    A  = B^{-1}A'B = \begin{pmatrix}
    
    0& 1   & & \\
     0&& 1 && \\
     0&&& \ddots & \\
     0&&& &1 \\
     a_{0} & a_{1} & \cdots & a_{n-2} & a_{n-1}\\
\end{pmatrix}
\end{equation}
  is the companion matrix for the polynomial $p_A(x) = x^{n} - a_{n-1} x^{n-1} - \cdots - a_0.$

Consider the vector $\bz = (z_0, \ldots, z_{n-1}).$ We can interpret $\bz$ as the coefficients of the polynomial $z(x) = z_{n-1} x^{n-1} + \ldots + z_0.$
Observe that the polynomial $z(x) x  \mod p_A(x)$ will have coefficient representation $\bz A$. In general $z(x) x^i$ will have coefficient representation given by $\bz A^i.$
The vector space $\Omega(\bz, A) \subseteq \Fq^n$ generated by $\bz, \bz A, \ldots, \bz A^{n-1}$ corresponds to the ideal generated by $z(x)$ in $\Fq[x]/p_A(x).$
This means that $\Omega(\bz,A)= \Fq^n$ if and only if $\gcd(z(x), p_A(x)) = 1.$
The probability of two monic polynomials in $\Fq[x]$ not both of degree zero to have no common divisor is $1- \frac{1}{q}$ \cite{Bennett07}.
From the proof in \cite{Bennett07} it is easy to see that this is also true if we consider the probability where one polynomial is monic of degree $n \geq 1$ and the other is a random polynomial (not necessarily monic) of degree less than $n$.


Consider $Z \in \Fq^{u \times n}$, and let $\Omega(Z,A) \subseteq \Fq^n$ be the space generated by the rows of $Z, ZA, \ldots, ZA^{n-1}.$
This space will correspond to the ideal of $\Fq[x]/p_A(x)$ generated by $z_1(x), \ldots, z_u(x)$ where $z_i(x)$ is the polynomial represented by the $i$-th row of $Z.$
The probability that $\Omega(Z,A) = \Fq^n$ correspond to the probability that $\gcd(p_A(x), z_1(x), \ldots, z_u(x)) = 1.$
The probability that $u+1$ monic polynomials of $\Fq[x]$ not all of degree zero have $\gcd$ equal to $1$ is estimated as $1-\frac{1}{q^u}$ \cite{Bennett07}.
Even in this case it is easy to see that the same result holds when we consider polynomials that are not necessarily monic or, as in our case, one polynomial is monic of degree $n \geq 1$ and the other polynomials are not necessarily monic of degree less than $n$.

For the uniformly distributed matrices $A$, Corollary \ref{cor:Pr(C_k^u)}
in Section \ref{sec:ExpRowSub} shows that the probability of $\Omega(Z,A) = \Fq^n$ is approximately $1-\frac{1}{(q-1)q^{u-1}}$.
It turns out that in the above extreme case, we obtain slightly better probability $1-\frac{1}{q^u}$.

% We expect that the intermediate cases will behave similarly to these two cases.
% In particular we expect them to be slightly worse than the companion matrix and slightly better than the uniform case.
% One reason to believe this is that matrices that are very bad are matrices who have lot of eigenvectors.
% An extreme case is represented by diagonal matrices which are included in the uniform case but are not in the other cases.
% Other examples of bad matrices are matrices that have a Frobenius normal form (also known as rational normal form) with small blocks on the diagonal.
% For the intermediate cases, the identity block in the lower left corner of $A$ guarantees that $\be_{(d-2)r - l} A^i = \be_{(d-2-i)r - l}$ for each $l<r.$
% As a consequence in the associated Frobenius normal form there will be several blocks of size at least $d-2.$
% In other words, the intermediate cases will avoid many "bad" matrices which are included in the uniform case.
% The fact that these bad cases are very uncommon among uniform matrices makes the difference between the two cases barely appreciable.


% To validate our hypothesis, in the first and third columns we report the expected values that should have been observed in the case that $Z,A$ were both chosen from a uniform distribution and in the case that $Z$ was chosen from a uniform distribution while $A$ was chosen uniformly from the companion matrices in $\Fq^{(d-1)r \times (d-1)r}$.
% The estimates we used for the first column derive from Corollary \ref{cor:Pr(C_k^u)} and corresponds to the probability $H_q(r(d-1) + u -1)/H_q(u-1)$.
% For the third column we used the probability $1 - q^{-u}$ which follows from the discussion in the previous paragraph.
% Notice that $r=1$ in the first example corresponds to a companion matrix while $d=2$ in the $5^{th}$ and $6^{th}$ examples corresponds to the uniform matrix case discussed in Section \ref{sec:ExpRowSub}.
% It is not a surprise that in these examples the measured value is close to the predicted value for the companion and uniform cases respectively. In the other examples we can observe how the measured value for $d>2, r>1$ always lies in between the two values predicted for the uniform and companion matrix cases which substantially confirms our hypothesis.

% Notice that, to an increase in the parameter $r,$ corresponds a measured value closer to the uniform distribution.
% Also notice that, for $q >2,$ the difference between what happens in the uniform and the companion matrix case becomes smaller.
% In particular for $q=3$ the difference is already considerably smaller than the case $q=2$ while, for $q=7$, the difference becomes negligible.
\cn

%
%The condition $\dim(\calV_{\alpha, d}.\calE) = dr$ is easy to satisfy. 
%When this condition is not satisfied, the problem to recover the product space becomes easier.
%The second condition depends strongly on the parameters. 
%Indeed if $d(n-k) > n$ it is not possible to satisfy this equation.
%For $d = 2$ both conditions seem reasonably easy to satisfy in most of the cases.
%Furthermore, for $d>2$,  
% While it is possible to give similar condition to Lemma \ref{lm:SyndromeUniform} for the case $d>2$, only the first $r$ rows of $A \in \Fq^{r(d-1) \times r(d-1)}$ can be considered as uniformly drawn but the remaining $(r-1)(d-1)$ are fixed.
% Even though $A$ is not uniform, 
%Although $A$ defined in \eqref{eq:matrix_A} cannot be considered to follow uniform distribution, experimental results show that the pairs $Z^{(1)}, A$ span the whole space $\Fq^{r(d-1)}$ with the same probability as given in Corollary \ref{cor:Pr(C_k^u)}.
%With the assumption that the pairs $Z^{(1)}, A$ behave like uniformly random distributed with respect to Corollary \ref{cor:Pr(C_k^u)}.

%\begin{proposition}\label{prop:2}
%Let $\calC \subseteq \Fqm^n $ be a BD-LRPC code having one 
%    parity-check matrix $H\in \Fqm^{(n-k)\times n}$ of support $\Span{\Fq}{H} = \calV_{\alpha, d}$ for some $\alpha \in \Fqm$ and a small integer $d\geq 2$. 
%    Suppose $\be\in\Fqm^n$ is an error of rank $r$ and denote $\calE=\Span{\Fq}{\be}$
%    and $\calS=\Span{\Fq}{\bs}$, where $\bs= \be H^\intercal$. Then, 
%    the probability that 
%    $\calV_{\alpha, r-1}.\calS = \calV_{\alpha, d+r-2}.\calE$ 
%    is given by $1-\frac{q+1}{q-1} q^{-u}$, where $u=(n-k)-r$. 
%\end{proposition}
%\begin{proof}
%    As it will be shown in Corollary \ref{cor:Pr(C_k^u)} in Section \ref{sec:ExpRowSub}, the probability that a matrix $\begin{psmallmatrix}  A \\ Z \end{psmallmatrix}$ uniformly drawn from $\Fq^{(r+u) \times r}$ leads to $\sum_{i=0}^{r-1} \RowSpan(ZA^{i}) = \Fq^r$ is in the order of $1 - \frac{q^{-u+1}}{q-1}.$ 
%At the same time, the probability that a random matrix $X_1$, uniformly chosen in $\Fq^{(r+u)\times r}$, has rank $r$ is given by 
%$$
%    q^{-(r+u)r}\prod_{i = 0}^{r-1}(q^{r+u} - q^i) \approx 1 - q^{-r-u} \sum_{i=0}^{r-1}q^i  \approx 1 - \frac{q^{-u}}{(q-1)}.
%$$
%Considering the two events as independent we obtain the claimed probability.
%\end{proof}




% To successfully correct an error $\be$ of rank $r$, the syndrome equation $H\be^\intercal = \bs^\intercal$ should satisfy $(n-k)dr \geq nr$, indicating $R\leq 1 - \frac{1}{d}$. 
% By properly choosing $u$, we obtain the following main theorem.
% \begin{theorem}\label{th:d2rate}
%     Let $\calC \subseteq \Fqm^n $ be an LRPC code having one 
%     parity-check matrice $H\in \Fqm^{(n-k)\times n}$ of support $\Span{\Fq}{H} = \calV$ for some $\alpha \in \Fqm$ and a small integer $d\geq 2$. 
%     For sufficiently large $m$, $n$ and $\delta \in (0,1)$,
%     when $u\geq n(\frac{1}{d}-\delta)$,
%     an error $\be\in\Fqm^n$ of rank $r=\delta n$ can be corrected with a failure rate in the order of $\frac{q^{-(u+1)}}{q-1}$ for a code rate 
%     $$
%     R = 1 - \delta - \frac{u}{n}.
%     $$
% \end{theorem}}
